How Robust is Unsupervised Representation Learning to Distribution Shift?

The robustness of machine learning algorithms to distributions shift is primarily discussed in the context of supervised learning (SL). As such, there is a lack of insight on the robustness of the representations learned from unsupervised methods, such as self-supervised learning (SSL) and auto-encoder based algorithms (AE), to distribution shift. We posit that the input-driven objectives of unsupervised algorithms lead to representations that are more robust to distribution shift than the target-driven objective of SL. We verify this by extensively evaluating the performance of SSL and AE on both synthetic and realistic distribution shift datasets. Following observations that the linear layer used for classification itself can be susceptible to spurious correlations, we evaluate the representations using a linear head trained on a small amount of out-of-distribution (OOD) data, to isolate the robustness of the learned representations from that of the linear head. We also develop "controllable" versions of existing realistic domain generalisation datasets with adjustable degrees of distribution shifts. This allows us to study the robustness of different learning algorithms under versatile yet realistic distribution shift conditions. Our experiments show that representations learned from unsupervised learning algorithms generalise better than SL under a wide variety of extreme as well as realistic distribution shifts.

==> 1introduction_v1.tex <==
\section{Introduction}

The in-distribution assumption between the train and test set of most machine learning datasets is harmful for developing machine learning systems for the real-world.
%
This is because the downstream tasks of machine learning models typically consist of data drawn from different distributions than the train set. 
%
To perform well on such out-of-distribution tasks requires the model to have good generalisation performance, which is not properly evaluated on standard machine learning datasets such as ImageNet, where the train and test set are sampled i.i.d. from the same distribution.

With the increasing attention on this issue, researchers have been probing the generalisation performance of models, setting up interesting datasets to examine distribution shift [CITE synthetic and real] and coming up with specialised algorithms that improves generalisation performance [CITE algorithms]. 
%
In this work, we identify the following problems in our current field and develop a suite of experiments to provide some solutions:


% \begin{itemize}[itemsep=1em,leftmargin=1em,labelwidth=*,align=left]
\vspace{-8pt}
\paragraph{Too many specialised supervised learning algorithms for distribution shift:}
%
% Not only does the type of datasets used to study distribution shift varies, this problem is also studied in multiple lines of work under terminologies such as simplicity bias [CITE], dataset bias [CITE], shortcut learning [CITE] that focus more on synthetic datasets, as well as domain generalistaion and robustness [CITE] that emphasise realistic datasets.
%
Distribution shift is studied in multiple areas of research, under terminologies such as simplicity bias [CITE], dataset bias [CITE], shortcut learning [CITE] and domain adaptation and generalisation [CITE].
%
Specialised algorithms are devised to improve generalisation performance, including methods that encourage the classifier to make invariant predictions across multiple data distributions [CITE], robust optimisation technique that minimises the worst case lost [CITE] as well as ensemble learning to avoid shortcut solution [CITE].

An important observation is that these specialised methods for generalisation are all developed under the supervised learning (SL) regime: strangely, popular unsupervised representation learning paradigm such as \gls{SSL} and \gls{AE} are largely overlooked in literature studying distribution shift.
%
This is particularly relevant because unsupervised learning regimes allows us to use large-scale unlabelled datasets, and we have seen evidence that training on more data is beneficial for OOD generalisation [CITE PRETRAINING STUDY, MEASURING ROBUSTNESS].
%
In addition, recent work has discovered that SL can be very susceptible to spurious correlation \citep{shah2020pitfalls, geirhos2020shortcut}, i.e. it is prone to learning features that are irrelevant to the true labelling functions yet highly predictive of the labels.
%
This behaviour of SL is not at all surprising if we consider its target-driven objective---when presented with two features that are equally predictive of the label, SL models have no incentive to learn both if learning only one of them suffice to accurately predict the target; if the OOD test set then relies on the feature that it ignores to make prediction, the generalisation performance of such a model will be very poor.
%
Therefore, considering unsupervised learning objectives has the additional benefit of potentially avoiding the pitfall of spurious correlation caused by target-driven objectives.

\emph{Our contribution:} We turn our attention to unsupervised pre-training methods, including \acrfull{SSL} algorithms~(e.g., \citep{chen2020simclr,grill2020byol,chen2021simsiam}), which learn representations by enforcing invariance between the representations of two distinctly augmented views of the same image,  and \acrfull{AE}~\citep{rumelhart1985ae,kingma2013vae,higgins2016betavae,burda2015iwae}, which learn by reconstructing the input image.
%
These methods have been under-explored in the context of distribution shift, and since \gls{SSL} and \gls{AE} methods do not require annotations of the data, we hypothesize that they stand a better chance at avoiding the exploitation of spurious correlation and thus faring better under distribution shift compared to \gls{SL}.

\vspace{-8pt}
\paragraph{Suboptimality of synthetic and realistic dataset:}
%
Datasets that study distribution shift can be summarised in two categories, namely synthetic datasets where the shift between train/test distribution is explicit and controlled [CITE dataset bias, spurious correlation, image corruption], and realistic datasets featuring distribution shift in the real world [CITE domain generalisation, imagenetv2 etc]. 
%
% However, even though both types of dataset set out to study OOD generalisation, there is a disconnection between the literature, with synthetic datasets appearing more in topics such as simplicity bias, dataset bias and spurious correlation [CITE dataset bias, spurious correlation, image corruption], while real-world datasets are emphasised in domain generalisation [CITE domain generalisation, imagenetv2 etc].
%
While realistic datasets are more reflective of naturally arising OOD generalisation scenarios, they do not serve as an effective diagnostic tool for generalisation performance. 
%
This is because the types of distribution shift featured in these datasets not only varies a lot, but are also subtle and hard to define. 
%
As a result, we typically see significant fluctuations in models' performance across datasets [CITE wilds], however we cannot explain what caused the change in performance.
%
% For instance, on WILDS benchmark with multiple datasets characterising domain generalisation in the wild, we see a variety of distribution shifts such as tissue scans from different hospitals, photos of animals captured in different locations and satellite images of different regions.
%
% If a model performs well on one of these datasets and poorly on another (which is often the case on WILDS benchmark), we have no way of understanding what caused the change in performance, making it difficult to determine when to use which model for deployment. 
%
With synthetic datasets, this becomes much easier as we are able to explicitly control the distribution shift, however the simplicit, toy-ish nature of these datasets poses scalibility concerns on the findings.

\emph{Our contribution:} In addition to evaluating models on both synthetic and realistic datasets, we subsample realistic domain generalisation datasets in WILDS to artificially create explicit correlation between domains and labels.
%
The resulting datasets both utilise real-world data and has distribution shift that is adjustable via the correlation coefficient between domain and label information.
%
By doing so, we are able to study distribution shift on complex, realistic data in a controlled environment, which allows us to draw convincing conclusions on models' behaviour under different settings.
%

\vspace{-8pt}
\paragraph{The significant bias of linear classifier head:} \citet{kang2019decoupling} and \citet{kirichenko2022last} observe the interesting phenomenon that the linear classifier itself is very susceptible to spurious correlation. They show that by simply retraining the linear classifier on data where the spurious correlation is removed, a model's performance can be drastically improved on the \gls{OOD} test set.
%
This indicates that the representations learned by the backbone of the model are able to capture \emph{both} the simple and the complex features in the data, however the linear classifier only assigns weights to those simpler features that are spuriously correlated to the labels.
%
While previous investigations of this effect focus mainly on synthetic data, it is possible that retraining the linear classifier head on OOD data could significantly improve the performance on real distribution shift problems as well\footnote{This is similar to linear probing in transfer learning setting.}.
%
Importantly, if our interest lies in examining how well the \emph{representations} learned from different models capture available features in the data (and thereby generalise better to unseen distributions), we should aim to isolate the bias of the linear classification head by retraining it on data drawn from the same distribution as the OOD test set.

\emph{Our contribution:} For all our experiments we report the performance using a linear head trained on \gls{OOD} data.
%
We also provide results using more standard evaluation scheme for distribution shift, where the linear head is trained on \gls{ID} data.
%
Note that in both scenarios, the model is evaluated on the \gls{OOD} test set. 

 


% A summary of the results using this methodology is presented in~\Cref{fig:summary}.
% %
% The evaluation with the \gls{OOD} linear head provides insight on whether the representations produced by the pre-trained models contain information about all features, and the difference between the \gls{ID} and \gls{OOD} linear head sheds light on the bias of the linear classifier.



In summary, we develop a suite of experiments  to evaluate the performance of various learning paradigm under distribution shift.~\Cref{fig:summary} provides a summary of our results, comparing a wide range of models from the following classes of methods:
%
\begin{enumerate*}[label=(\roman*)]
\item \gls{SSL},
\item \gls{AE}, and 
\item \gls{SL}.
\end{enumerate*}
%
To the best of our knowledge, we are the first to systematically evaluate the performance of these regimes under distribution shift.
%
In addition, to isolate the performance of the pre-trained models from the potential bias of the linear layer used for prediction, we establish a new evaluation scheme where the linear head is trained on \gls{OOD} data (right subplots in \cref{fig:ms_summary,fig:cdsprites_summary,fig:camelyon_summary}). We also provide results using the classical evaluation scheme, where the linear head is trained on \gls{ID} data (left subplots in \cref{fig:ms_summary,fig:cdsprites_summary,fig:camelyon_summary}). 
%
The models are evaluated on both synthetic and realistic distribution shift datasets, as well as subsampled realistic datasets that manufacture controllable, explicit spurious correlation.
%
The main takeaways from this paper are:

\begin{figure*}[t]
  \centering
  \captionsetup[subfigure]{belowskip=1ex}
  \begin{subfigure}{0.23\linewidth}
    \centering
    \includegraphics[width=0.48\linewidth]{images/intro_plot/mnist_cifar_summary_id_cifar.pdf}
    \includegraphics[width=0.48\linewidth]{images/intro_plot/mnist_cifar_summary_ood_cifar.pdf}
    \caption{MNIST-CIFAR} \label{fig:ms_summary}
  \end{subfigure}
  \begin{subfigure}{0.23\linewidth}
    \centering
    \includegraphics[width=0.48\linewidth]{images/intro_plot/cdsprites_summary_id_shape.pdf}
    \includegraphics[width=0.48\linewidth]{images/intro_plot/cdsprites_summary_ood_shape.pdf}
    \caption{CdSprites}\label{fig:cdsprites_summary}
  \end{subfigure}
  \begin{subfigure}{0.23\linewidth}
    \centering
    \includegraphics[width=0.48\linewidth]{images/intro_plot/linear_camelyon_summary_id_test.pdf}
    \includegraphics[width=0.48\linewidth]{images/intro_plot/linear_camelyon_summary_ood_test.pdf}
    \caption{Camelyon17}\label{fig:camelyon_summary}
  \end{subfigure}
  \begin{subfigure}{0.23\linewidth}
    \centering
    \includegraphics[width=0.48\linewidth]{images/intro_plot/linear_camelyon_corr100_summary_id_test.pdf}
    \includegraphics[width=0.48\linewidth]{images/intro_plot/linear_camelyon_corr100_summary_ood_test.pdf}
    \caption{Camelyon17\_SB}\label{fig:camelyon_sb_summary}
  \end{subfigure}    
  \vspace{-1em}
  \caption{OOD performance of auto-encoder based (AE), \acrfull{SSL}, \acrfull{SL} models. For each dataset, we evaluate on the OOD test set with linear heads trained on ID (left, transparent) and OOD data (right, solid) respectively. In each subplot, the lowest visible value corresponds to the relative frequency of the majority class from the respective dataset.}
  \label{fig:summary}
  \vspace{-12pt}
\end{figure*}



%
\begin{itemize}[nosep,leftmargin=1em,labelwidth=*,align=left]
   \item \textbf{\textit{Unsupervised learning models are generally more robust to distribution shift:}} Results of our proposed \gls{OOD} linear head evaluation show that \gls{SSL} models consistently achieve better performance than \gls{AE}, however, \gls{AE} models still perform at least as good as \gls{SL} on both synthetic and realistic settings that we study;
   \item \textbf{\textit{Performance of all models under both synthetic and realistic distribution shift can be significantly improved by retraining the last linear layer:}} We show a large performance gain evaluating the models using linear head trained on a small amount of OOD data, in contrast to the baseline where the linear head is trained on ID data (compare left to right subplots in \cref{fig:summary}); the surprising gain of this cheap procedure indicates that 1) existing pre-trained models, especially SSL, avoid the exploitation of spurious correlations and 2) more work on improving the performance under distribution shift should focus on balancing the final linear layer.
\end{itemize}




==> 1introduction_v2.tex <==
\section{Introduction} \label{sec:introduction}

The phenomenon where most of the train and test set of machine learning datasets follow the same distribution is harmful for the deployment of machine learning systems in the real world.
% The i.i.d. assumption between the train and test set of most machine learning datasets is harmful for developing machine learning systems for the real world.
%
This is because the downstream tasks of machine learning models typically consist of data drawn from different distributions than the train set. 
%
To perform well on such tasks requires the model to generalise well to unseen distributions, which is not investigated on standard, popular machine learning datasets such as ImageNet, where the train and test set are sampled i.i.d. from the same distribution.

With the increasing attention on this issue, researchers have been probing the generalisation performance of models by setting up datasets that feature distribution shift tasks \citep{koh2021wilds, domainbed, shah2020pitfalls} and proposing algorithms that aim to improve generalisation performance \citep{ganin2016dann, arjovsky2019irm, sun2016coral, Sagawa2020dro, fish}. 
%
In this work, we identify the several problems in this current field and develop a suite of experiments to address them --- see next section for more details.





==> 1introduction_v3.tex <==
\section{Introduction} \label{sec:introduction}

Machine Learning~(ML) algorithms are classically designed under the assumption that the training and test data are drawn from the same distribution. However, this assumption does not hold in most cases for the deployment of ML systems in the real world.
%
%However, this is potentially detrimental for the deployment of ML systems in the real world.
% The i.i.d. assumption between the train and test set of most machine learning datasets is harmful for developing machine learning systems for the real world.
%
% The downstream tasks, in which ML algorithms are deployed, typically
% operate in different environments than the one where the training data
% was drawn from. 
For example, medical researchers might obtain their training data from hospitals in Europe, but then deploy their trained models in Asia; the changes in conditions such as imaging equipment and demography result in a shift in the data distribution between train and test set~\citep{dockes2021preventing, glocker2019machine,henrich2010most}. 
% can arise due to multiple factors~\citep{dockes2021preventing}~e.g. changes in imaging equipment~\citep{glocker2019machine} and changes in demography~\citep{henrich2010most}.
% consist of data drawn from different distributions than the train
% set for various reasons including 
%
To perform well on such tasks requires the models to generalise well to unseen distributions --- an important property that is not evaluated on standard machine learning datasets like ImageNet, where the train and test set are sampled i.i.d. from the same distribution.

With the increasing attention on this issue, researchers have been probing the generalisation performance of ML models by creating datasets that feature distribution shift tasks~\citep{koh2021wilds, domainbed, shah2020pitfalls} and proposing algorithms that aim to improve generalisation performance under distribution shift~\citep{ganin2016dann, arjovsky2019irm, sun2016coral, Sagawa2020dro, fish}. 
%
In this work, we identify three specific problems with current approaches in distribution shift problems featuring image classification tasks, and develop a suite of experiments to address them.





==> 2backgrounds_v1.tex <==


\section{Existing problems and Contributions}
% \begin{itemize}[itemsep=1em,leftmargin=1em,labelwidth=*,align=left]
% \vspace{-8pt}
\paragraph{Problem 1: Too many specialised supervised learning algorithms for distribution shift.}
%
% Not only does the type of datasets used to study distribution shift varies, this problem is also studied in multiple lines of work under terminologies such as simplicity bias [CITE], dataset bias [CITE], shortcut learning [CITE] that focus more on synthetic datasets, as well as domain generalistaion and robustness [CITE] that emphasise realistic datasets.
%
Distribution shift is studied in multiple areas of research, under terminologies such as simplicity bias \citep{shah2020pitfalls, hermann2020shapes, kalimeris2019sgd, neyshabur2014search}, dataset bias \citep{torralba2011datasetbias1, kim2019datasetbias2, le2020datasetbias3}, shortcut learning \citep{geirhos2020shortcut} and domain adaptation and generalisation \citep{arjovsky2019irm, ganin2016dann, koh2021wilds, domainbed}.
%
Specialised algorithms are devised to improve generalisation performance, including methods that encourage the classifier to make invariant predictions across multiple data distributions \citep{arjovsky2019irm, ganin2016dann}, robust optimisation technique that minimises the worst case lost \citep{Sagawa2020dro} as well as ensemble learning to avoid shortcut solution \citep{teney2022evading}.

An important observation is that these specialised methods for generalisation are all developed under the supervised learning (SL) regime: strangely, popular unsupervised representation learning paradigm such as \acrfull{SSL} and \acrfull{AE} are largely overlooked in literature studying distribution shift.
%
We believe it is particularly meaningful to study the performance of these methods on distribution shift for the following reasons:
%
1) \gls{SSL} and \gls{AE} methods (and their extensions) have been achieving impressive representation learning performance \citep{chen2020simclr, grill2020byol, he2021mae, bao2021beit}, however they are mostly trained and tested on balanced, in-distribution test dataset;
%
2) neither SSL nor AE requires annotations, allowing for the possibility for them to be trained on very large-scale unlabelled datasets, which has been shown to be beneficial for OOD generalisation \citep{taori2020measuring, liu2022empirical};
%
3) SL is prone to learning features that are irrelevant to the true labelling functions yet highly predictive of the labels \citep{shah2020pitfalls, geirhos2020shortcut}.
%
This behaviour is unsurprising given its \emph{target-driven} objective (e.g. cross-entropy loss)---when presented with two features that are equally predictive of the label, SL models have no incentive to learn both if learning only one of them suffice to accurately predict the target; this could result in poor generalisation performance if the OOD test set relies on the overlooked feature.
%
Unsupervised learning objectives are in comparison more \emph{input-driven} (\citet{chen2020simclr,vib} shows that their objectives maxmises the mutual information between representations and input data), and therefore can potentially avoid the pitfall of spurious correlation.

\emph{\textbf{Contribution}: evaluate SSL and AE on distribution shift tasks.} We turn our attention to unsupervised pre-training methods, including \acrfull{SSL} algorithms~(e.g., \citep{chen2020simclr,grill2020byol,chen2021simsiam}), which learn representations by enforcing invariance between the representations of two distinctly augmented views of the same image,  and \acrfull{AE}~\citep{rumelhart1985ae,kingma2013vae,higgins2016betavae,burda2015iwae}, which learn by reconstructing the input image.
%
These methods have been under-explored in the context of distribution shift, and since \gls{SSL} and \gls{AE} methods do not require annotations of the data, we hypothesize that they stand a better chance at avoiding the exploitation of spurious correlation and thus faring better under distribution shift compared to \gls{SL}.

\vspace{-8pt}
\paragraph{Problem 2: Disconnection between synthetic and realistic dataset.}
%
Datasets that study distribution shift can be summarised in two categories, namely synthetic datasets where the shift between train/test distribution is explicit and controlled (e.g. Colored-MNIST \citep{arjovsky2019irm}, CdSprites \citep{fish}, MNIST-CIFAR \citep{shah2020pitfalls}), and realistic datasets featuring distribution shift in the real world (e.g. WILDS benchmark \citep{koh2021wilds}, ImageNetV2 \citep{recht2019imagenetv2}). 
%
We provide examples in \cref{fig:synthetic_v_real}.
%
However, even though both types of dataset set out to study OOD generalisation, their usage are commonly seen in two different sub-fields: typically, works that discuss simplicity bias, dataset bias and shortcut learning focus on synthetic datasets \citep{teney2022evading, shah2020pitfalls, ahn2022mitigating}, while those that propose new domain generalisation/adaptation algorithms emphasise evaluating their model on realistic datasets \citep{sun2016coral, ganin2016dann}.
%
While synthetic datasets provide an effective diagnostic tool for generalisation performance as they allow for explicit control of the distribution shift, the simplicit, toy-ish nature of these datasets poses generality concerns on the findings drawn from these experiments.
%
A model's robustness to simplicity bias on toy datasets is meaningless if it fails on similar real-world problems.
%
On the other hand, realistic datasets often feature distribution shifts that are subtle and hard to define.
%
As a result, models' performance typically fluctuates across datasets \citep{koh2021wilds, domainbed}, however we cannot explain what caused the change in results.

\emph{\textbf{Contribution}: controllable but realistic distribution shift tasks.} In addition to evaluating models on both synthetic and realistic datasets, we subsample realistic domain generalisation datasets in WILDS to artificially create explicit correlation between domains and labels.
%
The resulting datasets both utilise real-world data and has distribution shift that is adjustable via the correlation coefficient between domain and label information.
%
% By doing so, we are able to 1) discuss extreme simplicity bias under more realistic settings 2) study distribution shift on complex, realistic data in a controlled environment, which allows us to draw convincing conclusions on models' behaviour under different settings.
%
Note that there are datasets such as ImageNet-9, SVSF or Waterbirds that provide distribution shift controls for real images, however our sub-sampling of realistic domain generalisation datasets allow us to gain such control over distribution shift cheaply, and in addition provide further analysis on models' performance on these existing benchmarks.

\vspace{-8pt}
\paragraph{Problem 3: The significant bias of linear classifier head.} \citet{kang2019decoupling, menon2020overparameterisation, kirichenko2022last} observe the interesting phenomenon that the linear classifier itself is very susceptible to spurious correlation. They show that by simply retraining the linear classifier on data where the spurious correlation is removed, a model's performance can be drastically improved on the \gls{OOD} test set.
%
This indicates that the representations learned by the backbone of the model are able to capture \emph{both} the simple and the complex features in the data, however the linear classifier only assigns weights to those simpler features that are spuriously correlated to the labels.
%
While previous investigations of this effect focus mainly on synthetic data, it is possible that retraining the linear classifier head on OOD data could significantly improve the performance on real distribution shift problems as well\footnote{This is similar to linear probing in transfer learning setting.}.
%
Importantly, if our interest lies in examining how well the \emph{representations} learned from different models capture available features in the data (and thereby generalise better to unseen distributions), we should aim to isolate the bias of the linear classification head by retraining it on data drawn from the same distribution as the OOD test set.

\emph{\textbf{Contribution}: OOD linear head.} For all our experiments we report the performance using a linear head trained on \gls{OOD} data.
%
We also provide results using more standard evaluation scheme for distribution shift, where the linear head is trained on \gls{ID} data.
%
Note that in both scenarios, the model is evaluated on the \gls{OOD} test set. 

 






In summary, we develop a suite of experiments  to evaluate the performance of various learning paradigm under distribution shift.~\Cref{fig:summary} provides a summary of our results, comparing a wide range of models from the following classes of methods:
%
\begin{enumerate*}[label=(\roman*)]
\item \gls{SSL},
\item \gls{AE}, and 
\item \gls{SL}.
\end{enumerate*}
%
To the best of our knowledge, we are the first to systematically evaluate the performance of these regimes under distribution shift.
%
% In addition, to isolate the performance of the pre-trained models from the potential bias of the linear layer used for prediction, we establish a new evaluation scheme where the linear head is trained on \gls{OOD} data (right subplots in \cref{fig:ms_summary,fig:cdsprites_summary,fig:camelyon_summary}). We also provide results using the classical evaluation scheme, where the linear head is trained on \gls{ID} data (left subplots in \cref{fig:ms_summary,fig:cdsprites_summary,fig:camelyon_summary}). 
%
The models are evaluated on both synthetic and realistic distribution shift datasets, as well as subsampled realistic datasets that manufacture controllable, explicit spurious correlation.
%
The main takeaways from this paper are:

\begin{figure*}[t]
  \centering
  \captionsetup[subfigure]{belowskip=1ex}
%   \begin{minipage}{\linewidth}
%       \centering
%       OOD linear head $\aoco$
%   \end{minipage}
  \begin{subfigure}[t]{0.16\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/intro_plot/ms_acc.pdf}\\
    \includegraphics[width=\linewidth]{images/intro_plot/ms_rho.pdf}
    \caption{\scriptsize MNIST-CIFAR} \label{fig:ms_summary}
  \end{subfigure}
  \begin{subfigure}[t]{0.16\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/intro_plot/cdsprites_acc.pdf}\\
    \includegraphics[width=\linewidth]{images/intro_plot/cdsprites_rho.pdf}
    \caption{\scriptsize \centering CdSprites ($r_{\text{id}}=1$)}\label{fig:cdsprites_summary}
  \end{subfigure}
  \begin{subfigure}[t]{0.16\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/intro_plot/camelyon17_corr100_acc.pdf}\\
    \includegraphics[width=\linewidth]{images/intro_plot/camelyon17_corr100_rho.pdf}
    \caption{\scriptsize \centering Camelyon17-C\\ ($r_{\text{id}}=1$)}\label{fig:camelyon_c_summary}
  \end{subfigure}   
  \begin{subfigure}[t]{0.16\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/intro_plot/fmow_corr100_acc.pdf}\\
    \includegraphics[width=\linewidth]{images/intro_plot/fmow_corr100_rho.pdf}
    \caption{\scriptsize \centering FMoW-C\\ ($r_{\text{id}}=1$)}\label{fig:fmow_c_summary}
  \end{subfigure}  
  \begin{subfigure}[t]{0.16\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/intro_plot/camelyon17_corr0_acc.pdf}\\
    \includegraphics[width=\linewidth]{images/intro_plot/camelyon17_corr0_rho.pdf}
    \caption{\scriptsize Camelyon17}\label{fig:camelyon_summary}
  \end{subfigure}
  \begin{subfigure}[t]{0.16\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/intro_plot/fmow_corr0_acc.pdf}\\
    \includegraphics[width=\linewidth]{images/intro_plot/fmow_corr0_rho.pdf}
    \caption{\scriptsize FMoW}\label{fig:fmow_summary}
  \end{subfigure} 
  \vspace{-1em}
  \caption{Performance of auto-encoder based (AE), \acrfull{SSL}, \acrfull{SL} models. \textbf{\textit{Top row}}: the OOD test set accuracy using linear heads trained on OOD data; \textbf{\textit{Bottom row}}: the difference in accuracy between evaluation on ID test set vs. OOD test set (i.e. effective robustness, proposed by \citeauthor{taori2020measuring}). Higher is better.}
  \label{fig:summary}
  \vspace{-12pt}
\end{figure*}



%
\begin{itemize}[nosep,leftmargin=1em,labelwidth=*,align=left]
   \item \textbf{SSL and AE achieves stronger generalisation performance than SL under extreme distribution shift:}~\Cref{fig:ms_summary,fig:cdsprites_summary,fig:camelyon_c_summary,fig:fmow_c_summary} presents results on more challenging distribution shift scenario, where the training set exhibit some form of extreme spurious correlation. We see that for both synthetic and realistic datasets, SSL and AE consistently outperforms SL in terms of OOD accuracy;
   \item \textbf{SSL and AE's performance drop less under distribution shift than SL}: The effective robustness $\rho$ in \cref{fig:summary} evaluates the difference between ID and OOD accuracy, with larger $\rho$ indicating small performance drop under distribution shift. We see that the $\rho$ for SSL and AE are always much larger than SL's, indicating that their performance are more stable when moving from ID to OOD data, while for SL the drop can be as drastic as $48\%$ (\Cref{fig:ms_summary};
   \item \textbf{Performance of all models under both synthetic and realistic distribution shift can be significantly improved by retraining the last linear layer:} We show a large performance gain evaluating the models using linear head trained on a small amount of OOD data, in contrast to the baseline where the linear head is trained on ID data; the surprising gain of this cheap procedure even on realistic distribution shift problems indicates that more work on improving models' generalisation performance should focus on balancing the final linear layer.
\end{itemize}

==> 2backgrounds_v2.tex <==

\begin{figure*}[t]
  \centering
  \captionsetup[subfigure]{belowskip=1ex}
  \begin{minipage}{\linewidth}
      \centering
      OOD Accuracy (higher is better)
  \end{minipage}
  \begin{subfigure}[t]{0.16\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/intro_plot/ms_acc.pdf}
  \end{subfigure}
  \begin{subfigure}[t]{0.16\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/intro_plot/cdsprites_acc.pdf}
  \end{subfigure}
  \begin{subfigure}[t]{0.16\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/intro_plot/camelyon17_corr100_acc.pdf}
  \end{subfigure}   
  \begin{subfigure}[t]{0.16\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/intro_plot/fmow_corr100_acc.pdf}
  \end{subfigure}  
  \begin{subfigure}[t]{0.16\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/intro_plot/camelyon17_corr0_acc.pdf}
  \end{subfigure}
  \begin{subfigure}[t]{0.16\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/intro_plot/fmow_corr0_acc.pdf}
  \end{subfigure} 
  \begin{minipage}{\linewidth}
      \centering
      OOD Error - ID Error (lower is better)
  \end{minipage}  
  \begin{subfigure}[t]{0.16\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/intro_plot/ms_rho.pdf}
    \caption{\scriptsize MNIST-CIFAR} \label{fig:ms_summary}
  \end{subfigure}
  \begin{subfigure}[t]{0.16\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/intro_plot/cdsprites_rho_tba.pdf}
    \caption{\scriptsize \centering CdSprites ($r_{\text{id}}=1$)}\label{fig:cdsprites_summary}
  \end{subfigure}
  \begin{subfigure}[t]{0.16\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/intro_plot/camelyon17_corr100_rho.pdf}
    \caption{\scriptsize \centering Camelyon17-CS\\ ($r_{\text{id}}=1$)}\label{fig:camelyon_c_summary}
  \end{subfigure}   
  \begin{subfigure}[t]{0.16\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/intro_plot/fmow_corr100_rho.pdf}
    \caption{\scriptsize \centering FMoW-CS\\ ($r_{\text{id}}=1$)}\label{fig:fmow_c_summary}
  \end{subfigure}  
  \begin{subfigure}[t]{0.16\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/intro_plot/camelyon17_corr0_rho.pdf}
    \caption{\scriptsize Camelyon17}\label{fig:camelyon_summary}
  \end{subfigure}
  \begin{subfigure}[t]{0.16\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/intro_plot/fmow_corr0_rho.pdf}
    \caption{\scriptsize FMoW}\label{fig:fmow_summary}
  \end{subfigure} 
  
  \vspace{-1em}
  \caption{Performance of auto-encoder based (AE), \acrfull{SSL}, \acrfull{SL} models. \textbf{\textit{Top row}}: the OOD test set accuracy (\%) using linear heads trained on OOD data; \textbf{\textit{Bottom row}}: the difference in error rate  (\%) between evaluation on OOD test set vs. ID test set.}
  \label{fig:summary}
  \vspace{-12pt}
\end{figure*}

\section{Existing problems and Contributions}
% \begin{itemize}[itemsep=1em,leftmargin=1em,labelwidth=*,align=left]
% \vspace{-8pt}
\paragraph{Problem 1: The outdated focus on supervised regime for distribution shift.}
%
Distribution shift is studied in multiple areas of research, under terminologies such as simplicity bias \citep{shah2020pitfalls, neyshabur2014search}, dataset bias \citep{torralba2011datasetbias1}, shortcut learning \citep{geirhos2020shortcut} and domain adaptation and generalisation \citep{koh2021wilds, domainbed}.
%
However, most work are done under the supervised learning (SL) regime, including various works that either investigate spurious correlation \citep{shah2020pitfalls, hermann2020shapes, kalimeris2019sgd} or those that propose specialised methods to improve generalisation/avoid shortcut solutions \citep{arjovsky2019irm, ganin2016dann, Sagawa2020dro, teney2022evading}.

On the other hand, recent work has seen a surge of unsupervised representation learning algorithms such as \acrfull{SSL} and \acrfull{AE} \citep{chen2020simclr, grill2020byol, kingma2013vae, bao2021beit, he2021mae}.
%
Their impressive performance on various tasks led to their popularisation, however these methods are mostly known for their strong performance tested on balanced, \gls{ID} test dataset --- how they perform on distribution shift tasks remains largely unknown.
%
We believe it is particularly meaningful to study the performance of these methods on distribution shift tasks for the following reasons:
%
\begin{enumerate}[nosep,leftmargin=1em,labelwidth=*,align=left]
   \item Neither SSL nor AE requires annotations, allowing for the possibility for them to be trained on very large-scale unlabelled datasets, which has been shown to be beneficial for OOD generalisation \citep{taori2020measuring, liu2022empirical};
   \item SL is prone to learning features that are irrelevant to the true labelling functions yet highly predictive of the labels \citep{shah2020pitfalls, geirhos2020shortcut}.
   %
   This behaviour is unsurprising given its \emph{target-driven} objective (e.g. cross-entropy loss)---when presented with two features that are equally predictive of the label, SL models have no incentive to learn both if learning only one of them suffice to accurately predict the target; this could result in poor generalisation performance if the OOD test set relies on the overlooked feature.
   %
   Unsupervised learning objectives are in comparison more \emph{input-driven} (\citet{chen2020simclr,vib} shows that their objectives maxmises the mutual information between representations and input data), and therefore can potentially avoid the pitfall of spurious correlation.
\end{enumerate}

\emph{\textbf{Contribution}: Evaluate SSL and AE on distribution shift tasks.} We turn our attention to unsupervised pre-training methods, including \gls{SSL} algorithms~(e.g., \citep{chen2020simclr,grill2020byol,chen2021simsiam}), which learn representations by enforcing invariance between the representations of two distinctly augmented views of the same image,  and \gls{AE}~\citep{rumelhart1985ae,kingma2013vae,higgins2016betavae,burda2015iwae}, which learn by reconstructing the input image.
%
These methods have been under-explored in the context of distribution shift, and since \gls{SSL} and \gls{AE} methods do not require annotations of the data, we hypothesize that they stand a better chance at avoiding the exploitation of spurious correlation and thus faring better under distribution shift compared to \gls{SL}.

\vspace{-8pt}
%
\paragraph{Problem 2: Disconnection between synthetic and realisitc datasets.}
%
Datasets that study distribution shift can be summarised in two categories, namely synthetic datasets where the shift between train/test distribution is explicit and controlled (e.g. MNIST-CIFAR \citep{shah2020pitfalls}, CdSprites \citep{fish}), and realistic datasets featuring distribution shift in the real world (e.g. WILDS \citep{koh2021wilds}). 
%
We provide examples in \cref{fig:synthetic_v_real}.
%
% However, even though both types of dataset sets out to study OOD generalisation, their usage are commonly seen in two different sub-fields: typically, works that discuss simplicity bias, dataset bias and shortcut learning focus on synthetic datasets \citep{teney2022evading, shah2020pitfalls, ahn2022mitigating}, while those that propose new domain generalisation/adaptation algorithms emphasise evaluating their model on realistic datasets \citep{sun2016coral, ganin2016dann}.

While synthetic datasets allow for explicit control of the distribution shift and therefore provide an effective diagnostic tool for generalisation performance, the simplicit nature of these datasets poses generality concerns on the findings drawn from these experiments:
%
a model's robustness to spurious correlation on toy datasets is meaningless if it fails on similar real-world problems.
%
On the other hand, realistic datasets often feature distribution shifts that are subtle, hard to define that also vary with task (see \cref{fig:synthetic_v_real}, right).
%
As a result, models' performance fluctuates a lot across datasets \citep{koh2021wilds, domainbed}, however we cannot explain what caused the change in results.

\begin{figure*}[t]
    \centering
    \includegraphics[trim={0.5cm 0 0 0},clip, width=\linewidth]{images/hook.png}
    \vspace{-2em}
    \caption{\textbf{Synthetic vs. realistic distribution shift:} The distribution shift in synthetic datasets (\textit{left}, MNIST-CIFAR and CdSprites) are usually extreme and controllable (adjusted via changing the correlation); for realistic datasets (\textit{right}, WILDS-Camelyon17 and FMoW) distribution shift can be subtle, hard to identify and impossible to control.}
    \vspace{-20pt}
    \label{fig:synthetic_v_real}
\end{figure*}

\emph{\textbf{Contribution}: Controllable but realistic distribution shift tasks.} In addition to evaluating models on both synthetic and realistic datasets, we subsample realistic domain generalisation datasets in WILDS to artificially create explicit correlation between domains and labels.
%
The resulting datasets both utilise real-world data and has distribution shift that is adjustable via the correlation coefficient between domain and label information.
%
Note that there are datasets such as ImageNet-9, SVSF or Waterbirds that provide distribution shift controls for real images, however our sub-sampling of realistic domain generalisation datasets allow us to gain such control over distribution shift cheaply, and in addition provide further analysis on models' performance on these existing benchmarks.

\vspace{-8pt}
\paragraph{Problem 3: The strong bias of linear classifier head.} \citet{kang2019decoupling, menon2020overparameterisation, kirichenko2022last} observe the interesting phenomenon that the linear classifier itself is very susceptible to spurious correlation. They show that by simply retraining the linear classifier on data where the spurious correlation is removed, a model's performance can be drastically improved on the \gls{OOD} test set.
%
This indicates that the representations learned by the backbone of the model are able to capture \emph{both} the simple and the complex features in the data, however the linear classifier only assigns weights to those simpler features that are spuriously correlated to the labels.
%
While previous investigations of this effect focus mainly on synthetic data, it is possible that retraining the linear classifier head on OOD data could significantly improve the performance on real distribution shift problems as well\footnote{This is similar to linear probing in transfer learning setting.}.
%
Importantly, if our interest lies in examining how well the \emph{representations} learned from different objectives capture available features in the data (and thereby generalise better to unseen distributions), we should aim to isolate the bias of the linear classification head by retraining it on data drawn from the same distribution as the OOD test set.

\emph{\textbf{Contribution}: OOD linear head.} For all our experiments we report the generalisation performance using a linear head trained on \gls{OOD} data.
%
We also quantify the linear head bias by comparing this value to the performance using linear head trained on \gls{ID} data.

 




In summary, we develop a suite of experiments  to evaluate the performance of various learning paradigm under distribution shift.~\Cref{fig:summary} provides a summary of our results, comparing a wide range of algorithms from the following classes of objectives:
%
\begin{enumerate*}[label=(\roman*)]
\item \gls{SSL},
\item \gls{AE}, and 
\item \gls{SL}.
\end{enumerate*}
%
To the best of our knowledge, we are the first to systematically evaluate the performance of these regimes under distribution shift.
%
% In addition, to isolate the performance of the pre-trained models from the potential bias of the linear layer used for prediction, we establish a new evaluation scheme where the linear head is trained on \gls{OOD} data (right subplots in \cref{fig:ms_summary,fig:cdsprites_summary,fig:camelyon_summary}). We also provide results using the classical evaluation scheme, where the linear head is trained on \gls{ID} data (left subplots in \cref{fig:ms_summary,fig:cdsprites_summary,fig:camelyon_summary}). 
%
The models are evaluated on both synthetic and realistic distribution shift datasets, as well as subsampled realistic datasets that manufacture controllable, explicit spurious correlation.
%
The main takeaways from this paper are:











% \begin{figure*}[t]
%   \centering
%   \captionsetup[subfigure]{belowskip=1ex}
% %   \begin{minipage}{\linewidth}
% %       \centering
% %       OOD linear head $\aoco$
% %   \end{minipage}
%   \begin{subfigure}[t]{0.16\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{images/intro_plot/ms_acc.pdf}\\
%     \includegraphics[width=\linewidth]{images/intro_plot/ms_rho.pdf}
%     \caption{\scriptsize MNIST-CIFAR} \label{fig:ms_summary}
%   \end{subfigure}
%   \begin{subfigure}[t]{0.16\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{images/intro_plot/cdsprites_acc.pdf}\\
%     \includegraphics[width=\linewidth]{images/intro_plot/cdsprites_rho_tba.pdf}
%     \caption{\scriptsize \centering CdSprites ($r_{\text{id}}=1$)}\label{fig:cdsprites_summary}
%   \end{subfigure}
%   \begin{subfigure}[t]{0.16\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{images/intro_plot/camelyon17_corr100_acc.pdf}\\
%     \includegraphics[width=\linewidth]{images/intro_plot/camelyon17_corr100_rho.pdf}
%     \caption{\scriptsize \centering Camelyon17-C\\ ($r_{\text{id}}=1$)}\label{fig:camelyon_c_summary}
%   \end{subfigure}   
%   \begin{subfigure}[t]{0.16\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{images/intro_plot/fmow_corr100_acc.pdf}\\
%     \includegraphics[width=\linewidth]{images/intro_plot/fmow_corr100_rho.pdf}
%     \caption{\scriptsize \centering FMoW-C\\ ($r_{\text{id}}=1$)}\label{fig:fmow_c_summary}
%   \end{subfigure}  
%   \begin{subfigure}[t]{0.16\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{images/intro_plot/camelyon17_corr0_acc.pdf}\\
%     \includegraphics[width=\linewidth]{images/intro_plot/camelyon17_corr0_rho.pdf}
%     \caption{\scriptsize Camelyon17}\label{fig:camelyon_summary}
%   \end{subfigure}
%   \begin{subfigure}[t]{0.16\linewidth}
%     \centering
%     \includegraphics[width=\linewidth]{images/intro_plot/fmow_corr0_acc.pdf}\\
%     \includegraphics[width=\linewidth]{images/intro_plot/fmow_corr0_rho.pdf}
%     \caption{\scriptsize FMoW}\label{fig:fmow_summary}
%   \end{subfigure} 
%   \vspace{-1em}
%   \caption{Performance of auto-encoder based (AE), \acrfull{SSL}, \acrfull{SL} models. \textbf{\textit{Top row}}: the OOD test set accuracy using linear heads trained on OOD data; \textbf{\textit{Bottom row}}: the difference in accuracy between evaluation on ID test set vs. OOD test set (i.e. effective robustness, proposed by \citeauthor{taori2020measuring}). Higher is better.}
%   \label{fig:summary}
%   \vspace{-12pt}
% \end{figure*}



%
\begin{itemize}[nosep,leftmargin=1em,labelwidth=*,align=left]
   \item \textbf{SSL and AE are more robust than SL to extreme distribution shift:}~\Cref{fig:ms_summary,fig:cdsprites_summary,fig:camelyon_c_summary,fig:fmow_c_summary} presents results on more challenging distribution shift scenario, where the training set exhibit some form of extreme spurious correlation. For both synthetic (\Cref{fig:ms_summary,fig:cdsprites_summary}) and realistic (\Cref{fig:camelyon_c_summary,fig:fmow_c_summary}) datasets, SSL and AE consistently outperforms SL in terms of OOD accuracy (top row); 
   \item \textbf{SSL and AE's performance drop less under distribution shift than SL}: The bottom row of~\Cref{fig:summary} reports the difference between ID and OOD accuracy (i.e. $\rho$, see \cref{sec:setup} for definition). Larger values are desirable, as they indicate less performance drop when evaluating on OOD data. Results show that SSL and AE's are significantly more stable under distribution shift  than SL;
   \item \textbf{Generalisation performance on realistic distribution shift task can be significantly improved by retraining the last linear layer:} We show a large performance gain evaluating all models using linear head trained on a small amount of OOD data, in contrast to the baseline where the linear head is trained on ID data; the surprising gain of this cheap procedure even on realistic distribution shift problems indicates that more work on improving models' generalisation performance should focus on balancing the final linear layer.
\end{itemize}

==> 2backgrounds_v3.tex <==

\begin{figure*}[t]
  \centering
  \captionsetup[subfigure]{belowskip=1ex}
  \begin{minipage}{\linewidth}
      \centering
      OOD Accuracy (higher is better)
  \end{minipage}
  \begin{subfigure}[t]{0.16\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/intro_plot/ms_acc.pdf}
  \end{subfigure}
  \begin{subfigure}[t]{0.16\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/intro_plot/cdsprites_summary_ood_shape.pdf}
  \end{subfigure}
  \begin{subfigure}[t]{0.16\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/intro_plot/camelyon17_corr100_acc.pdf}
  \end{subfigure}   
  \begin{subfigure}[t]{0.16\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/intro_plot/fmow_corr100_acc.pdf}
  \end{subfigure}  
  \begin{subfigure}[t]{0.16\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/intro_plot/camelyon17_corr0_acc.pdf}
  \end{subfigure}
  \begin{subfigure}[t]{0.16\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/intro_plot/fmow_corr0_acc.pdf}
  \end{subfigure} 
  \begin{minipage}{\linewidth}
      \centering
      OOD Error - ID Error (lower is better)
  \end{minipage}  
  \begin{subfigure}[t]{0.15\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/intro_plot/ms_rho.pdf}
    \caption{\scriptsize MNIST-CIFAR} \label{fig:ms_summary}
  \end{subfigure}
  \begin{subfigure}[t]{0.15\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/intro_plot/cdsprites_summary_rho.pdf}
    \caption{\scriptsize \centering CdSprites ($r_{\text{id}}=1$)}\label{fig:cdsprites_summary}
  \end{subfigure}
  \begin{subfigure}[t]{0.18\linewidth}
    \centering
    \includegraphics[width=0.833\linewidth]{images/intro_plot/camelyon17_corr100_rho.pdf}
    \caption{\scriptsize \centering Camelyon17-CS ($r_{\text{id}}=1$)}
    \label{fig:camelyon_c_summary}
  \end{subfigure}   
  \begin{subfigure}[t]{0.15\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/intro_plot/fmow_corr100_rho.pdf}
    \caption{\scriptsize \centering FMoW-CS ($r_{\text{id}}=1$)}\label{fig:fmow_c_summary}
  \end{subfigure}  
  \begin{subfigure}[t]{0.15\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/intro_plot/camelyon17_corr0_rho.pdf}
    \caption{\scriptsize Camelyon17}\label{fig:camelyon_summary}
  \end{subfigure}
  \begin{subfigure}[t]{0.15\linewidth}
    \centering
    \includegraphics[width=\linewidth]{images/intro_plot/fmow_corr0_rho.pdf}
    \caption{\scriptsize FMoW}\label{fig:fmow_summary}
  \end{subfigure} 
  
  \vspace{-1em}
  \caption{Performance of auto-encoder based (AE), \acrfull{SSL}, \acrfull{SL} models. \textbf{\textit{Top row}}: the OOD test set accuracy (\%) using linear heads trained on OOD data; \textbf{\textit{Bottom row}}: the difference in error rate  (\%) between evaluation on OOD test set vs. ID test set.}
  \label{fig:summary}
  \vspace{-12pt}
\end{figure*}

\section{Existing problems and Contributions} \label{sec:background}
% \begin{itemize}[itemsep=1em,leftmargin=1em,labelwidth=*,align=left]
% \vspace{-8pt}
\paragraph{Problem 1: The outdated focus on supervised regime for distribution shift.}
%
Distribution shift is studied in multiple areas of research, under terminologies such as simplicity bias \citep{shah2020pitfalls}, dataset bias \citep{torralba2011datasetbias1}, shortcut learning \citep{geirhos2020shortcut} and domain adaptation and generalisation \citep{koh2021wilds, domainbed}.
%
However, most work are done under the supervised learning (SL) regime, including various works that either investigate spurious correlation \citep{shah2020pitfalls, hermann2020shapes, kalimeris2019sgd} or those that propose specialised methods to improve generalisation/avoid shortcut solutions \citep{arjovsky2019irm, ganin2016dann, Sagawa2020dro, teney2022evading}.

On the other hand, recent work has seen a surge of unsupervised representation learning algorithms such as \acrfull{SSL}~(e.g., \citep{chen2020simclr,grill2020byol,chen2021simsiam}), which learn representations by enforcing invariance between the representations of two distinctly augmented views of the same image,  and \acrfull{AE}~\citep{rumelhart1985ae,kingma2013vae,higgins2016betavae,burda2015iwae}, which learn by reconstructing the input image.
% such as \acrfull{SSL} and \acrfull{AE} \citep{chen2020simclr, grill2020byol, kingma2013vae, bao2021beit, he2021mae}.
%
Their impressive performance on various tasks led to their popularisation, however these methods are mostly known for their strong performance tested on balanced, \gls{ID} test dataset --- how they perform on distribution shift tasks remains largely unknown.
%
We believe it is particularly meaningful to study the \acrfull{OOD} generalisation performance of these unsupervised methods, as recent research has point out that SL is very vulnerable to spurious correlation, and is prone to learning \emph{only} features that are irrelevant to the true labelling functions yet highly predictive of the labels \citep{shah2020pitfalls, geirhos2020shortcut}.
%
This can result in poor performance on \gls{OOD} test set, if the spurious feature learned by the model is no longer presented.
%
This behaviour is unsurprising given SL's \emph{target-driven} objective (e.g. cross-entropy loss)---when presented with two features that are equally predictive of the label, SL models have no incentive to learn both if learning only one of them suffice to accurately predict the target; 
%
the choice then comes down to the inductive bias of the optimiser and the model architecture.
% this could result in poor generalisation performance if the OOD test set relies on the overlooked feature.
%
Unsupervised learning objectives are in comparison more \emph{input-driven}, i.e. they learn to  maxmise the mutual information between representations and input data \citet{chen2020simclr,vib}.
%
We hypothesise that this characteristic of unsupervised objectives gives them a better chance to avoid the exploitation of spurious correlation, and thus faring better under distribution shift compared to SL.

\emph{\textbf{Contribution}: Evaluate SSL and AE on distribution shift tasks.} We evaluate and compare the generalisation performance of unsupervised methods, including \gls{SSL} and \gls{AE}, to standard supervised learning. See \cref{sec:setup} for more details.

\vspace{-8pt}
%
\paragraph{Problem 2: Disconnection between synthetic and realisitc datasets.}
%
There are two types of datasets that study distribution shift: synthetic datasets where the shift between train/test distribution is explicit and controlled (e.g. MNIST-CIFAR \citep{shah2020pitfalls}, CdSprites \citep{fish}), and realistic datasets featuring distribution shift in the real world (e.g. WILDS \citep{koh2021wilds}). 
%
We provide examples in \cref{fig:synthetic_v_real}.
%
% However, even though both types of dataset sets out to study OOD generalisation, their usage are commonly seen in two different sub-fields: typically, works that discuss simplicity bias, dataset bias and shortcut learning focus on synthetic datasets \citep{teney2022evading, shah2020pitfalls, ahn2022mitigating}, while those that propose new domain generalisation/adaptation algorithms emphasise evaluating their model on realistic datasets \citep{sun2016coral, ganin2016dann}.

While synthetic datasets allow for explicit control of the distribution shift and therefore provide an effective diagnostic tool for generalisation performance, the simplicit nature of these datasets poses concerns of generality on the findings drawn from these experiments:
%
a model's robustness to spurious correlation on toy datasets is meaningless if it fails on similar real-world problems.
%
On the other hand, realistic datasets often feature distribution shifts that are subtle, hard to define that vary with task (see \cref{fig:synthetic_v_real}, right).
%
As a result, models' performance tend to fluctuate across datasets \citep{koh2021wilds, domainbed}, while the cause of such fluctuations remains unknown.

% however we cannot explain what caused the change in results.

\begin{figure*}[t]
    \centering
    \includegraphics[trim={0.5cm 0 0 0},clip, width=\linewidth]{images/hook.png}
    \vspace{-2em}
    \caption{\textbf{Synthetic vs. realistic distribution shift:} The distribution shift in synthetic datasets (\textit{left}, MNIST-CIFAR and CdSprites) are usually extreme and controllable (adjusted via changing the correlation); for realistic datasets (\textit{right}, WILDS-Camelyon17 and FMoW) distribution shift can be subtle, hard to identify and impossible to control.}
    \vspace{-20pt}
    \label{fig:synthetic_v_real}
\end{figure*}

\emph{\textbf{Contribution}: Controllable but realistic distribution shift tasks.} In addition to evaluating models on both synthetic and realistic datasets, we subsample realistic domain generalisation datasets in WILDS to artificially create explicit correlation between domains and labels.
%
The resulting datasets both utilise real-world data and has distribution shift that is adjustable via the correlation coefficient between domain and label information.
%
Note that there are datasets such as ImageNet-9, SVSF or Waterbirds that provide distribution shift controls for real images, however our sub-sampling of realistic domain generalisation datasets allow us to gain such control over distribution shift cheaply, and in addition provide further analysis on models' performance on these existing benchmarks.

\vspace{-8pt}
\paragraph{Problem 3: The strong bias of linear classifier head.} \citet{kang2019decoupling, menon2020overparameterisation} observe the interesting phenomenon that the final layer linear classifier of deep learning models is very susceptible to spurious correlation, and therefore a strong source of model bias. They show that by simply retraining the linear classifier on data where the spurious correlation is removed, a model's performance on OOD test set can be drastically improved.
%
This indicates that the representations learned by the backbone of the model are able to faithfully capture different features available in the input data, however the linear classifier only assign weights to some of those features (usually the simpler ones) that are spuriously correlated to the labels.
%
While previous investigations of this effect focus mainly on synthetic data, it is possible that retraining the linear classifier head on OOD data could also improve the performance on real distribution shift problems
% \footnote{This is similar to linear probing in transfer learning setting.}.
%
Importantly, if our interest lies in examining how well the \emph{representations} learned from different objectives capture available features in the data (and thereby generalise better to unseen distributions), we should aim to isolate the bias of the linear classification head by retraining it on data drawn from the same distribution as the OOD test set.

\emph{\textbf{Contribution}: OOD linear head.} For all our experiments we report the OOD accuracy using a linear head trained on small amount of left-out \gls{OOD} data.
%
We also quantify the linear head bias to highlight the importance of this treatment when evaluating generalisation performance. 
% More details in \cref{sec:setup}.

 

In summary, we develop a suite of experiments  to evaluate the performance of various learning paradigm under distribution shift.~\Cref{fig:summary} provides a summary of our results, comparing a wide range of algorithms from the following classes of objectives:
%
\begin{enumerate*}[label=(\roman*)]
\item \gls{SSL},
\item \gls{AE}, and 
\item \gls{SL}.
\end{enumerate*}
%
To the best of our knowledge, we are the first to systematically evaluate the performance of these regimes under distribution shift.
%
The models are evaluated on both synthetic and realistic distribution shift datasets, as well as subsampled realistic datasets that manufacture controllable, explicit spurious correlation.
%
The main takeaways from this paper are:


%
\begin{itemize}[nosep,leftmargin=1em,labelwidth=*,align=left]
   \item \textbf{SSL and AE are more robust than SL to extreme distribution shift:}~\Cref{fig:ms_summary,fig:cdsprites_summary,fig:camelyon_c_summary,fig:fmow_c_summary} presents results on more challenging distribution shift scenario, where the training set exhibit some form of extreme spurious correlation. For both synthetic (\Cref{fig:ms_summary,fig:cdsprites_summary}) and realistic (\Cref{fig:camelyon_c_summary,fig:fmow_c_summary}) datasets, SSL and AE consistently outperforms SL in terms of OOD accuracy (top row); 
   \item \textbf{SSL and AE's performance drop less under distribution shift than SL}: The bottom row of \cref{fig:summary} reports the difference between ID and OOD accuracy (i.e. shift sensitivity $s$, see \cref{sec:setup} for definition). Smaller $s$ is desirable as it indicates lower sensitivity to distribution shift. Results show that SSL and AE's are significantly more stable under distribution shift  than SL;
   \item \textbf{Generalisation performance on realistic distribution shift task can be significantly improved by retraining the last linear layer:} We show a large performance boost evaluating all models using linear head trained on a small amount of OOD data, in contrast to the baseline where the linear head is trained on ID data; the surprising gain of this cheap procedure even on realistic distribution shift problems highlights the importance of isolating the linear head bias when evaluating models' generalisation performance.
\end{itemize}

==> 2backgrounds_v4.tex <==

\begin{figure*}[t]
    \centering
    \captionsetup[subfigure]{belowskip=1ex}
    \begin{minipage}{\linewidth}
        \centering
        OOD Accuracy (higher is better)
    \end{minipage}
    \begin{subfigure}[t]{0.16\linewidth}
      \centering
      \includegraphics[width=\linewidth]{images/intro_plot/ms_acc.pdf}
    \end{subfigure}
    \begin{subfigure}[t]{0.16\linewidth}
      \centering
      \includegraphics[width=\linewidth]{images/intro_plot/cdsprites_summary_ood_shape.pdf}
    \end{subfigure}
    \begin{subfigure}[t]{0.16\linewidth}
      \centering
      \includegraphics[width=\linewidth]{images/intro_plot/camelyon17_corr100_acc.pdf}
    \end{subfigure}   
    \begin{subfigure}[t]{0.16\linewidth}
      \centering
      \includegraphics[width=\linewidth]{images/intro_plot/fmow_corr100_acc.pdf}
    \end{subfigure}  
    \begin{subfigure}[t]{0.16\linewidth}
      \centering
      \includegraphics[width=\linewidth]{images/intro_plot/camelyon17_corr0_acc.pdf}
    \end{subfigure}
    \begin{subfigure}[t]{0.16\linewidth}
      \centering
      \includegraphics[width=\linewidth]{images/intro_plot/fmow_corr0_acc.pdf}
    \end{subfigure} 
    \begin{minipage}{\linewidth}
        \centering
        OOD Error - ID Error (lower is better)
    \end{minipage}  
    \begin{subfigure}[t]{0.15\linewidth}
      \centering
      \includegraphics[width=\linewidth]{images/intro_plot/ms_rho.pdf}
      \caption{\scriptsize MNIST-CIFAR} \label{fig:ms_summary}
    \end{subfigure}
    \begin{subfigure}[t]{0.15\linewidth}
      \centering
      \includegraphics[width=\linewidth]{images/intro_plot/cdsprites_summary_rho.pdf}
      \caption{\scriptsize \centering CdSprites ($r_{\text{id}}=1$)}\label{fig:cdsprites_summary}
    \end{subfigure}
    \begin{subfigure}[t]{0.18\linewidth}
      \centering
      \includegraphics[width=0.838\linewidth]{images/intro_plot/camelyon17_corr100_rho.pdf}
      \caption{\scriptsize \centering Camelyon17-CS ($r_{\text{id}}=1$)}
      \label{fig:camelyon_c_summary}
    \end{subfigure}   
    \begin{subfigure}[t]{0.15\linewidth}
      \centering
      \includegraphics[width=\linewidth]{images/intro_plot/fmow_corr100_rho.pdf}
      \caption{\scriptsize \centering FMoW-CS ($r_{\text{id}}=1$)}\label{fig:fmow_c_summary}
    \end{subfigure}  
    \begin{subfigure}[t]{0.15\linewidth}
      \centering
      \includegraphics[width=\linewidth]{images/intro_plot/camelyon17_corr0_rho.pdf}
      \caption{\scriptsize Camelyon17}\label{fig:camelyon_summary}
    \end{subfigure}
    \begin{subfigure}[t]{0.15\linewidth}
      \centering
      \includegraphics[width=\linewidth]{images/intro_plot/fmow_corr0_rho.pdf}
      \caption{\scriptsize FMoW}\label{fig:fmow_summary}
    \end{subfigure} 
    
    \vspace{-1em}
    \caption{Performance of auto-encoder based (AE), \acrfull{SSL}, \acrfull{SL} models. \textbf{\textit{Top row}}: the OOD test set accuracy (\%) using linear heads trained on OOD data; \textbf{\textit{Bottom row}}: the difference in error rate  (\%) between evaluation on OOD test set vs. ID test set.}
    \label{fig:summary}
    \vspace{-12pt}
  \end{figure*}
  
  \subsection{Existing problems and Contributions} \label{sec:background}
  % \begin{itemize}[itemsep=1em,leftmargin=1em,labelwidth=*,align=left]
  % \vspace{-8pt}
  \paragraph{Problem 1: The outdated focus on supervised regime for distribution shift}
  %
  In ML research, distribution shfit is studied under varied
  terminologies such as simplicity bias~\citep{shah2020pitfalls},
  dataset bias~\citep{torralba2011datasetbias1}, shortcut
  learning~\citep{geirhos2020shortcut}, and domain adaptation and
  generalisation \citep{koh2021wilds, domainbed}.
  %
  However, most of them are done in the regime of supervised learning
  (SL), including various works that either investigate
  spurious correlations~\citep{shah2020pitfalls, hermann2020shapes,
  kalimeris2019sgd} or those that propose specialised methods to
  improve generalisation and/or avoid shortcut solutions~\citep{arjovsky2019irm, ganin2016dann, Sagawa2020dro,
  teney2022evading}.
  
  On the other hand, recent work in representation learning of images has seen a surge of unsupervised learning algorithms such as \acrfull{SSL}~(e.g., \citet{chen2020simclr,grill2020byol,chen2021simsiam}), which learn representations by enforcing invariance between the representations of two distinctly augmented views of the same image,  and \acrfull{AE}~\citet{rumelhart1985ae,kingma2013vae,higgins2016betavae,burda2015iwae}, which learn by reconstructing the input image.
  % such as \acrfull{SSL} and \acrfull{AE} \citep{chen2020simclr, grill2020byol, kingma2013vae, bao2021beit, he2021mae}.
  %
  While their impressive performance on various tasks led to their
  popularisation, these methods are mostly known for their
  strong performance on balanced \gls{ID} test datasets --- how they
  perform on distribution shift tasks remains largely unknown. 
  %
  We believe it is particularly meaningful to study the \acrfull{OOD}
  generalisation performance of the representations learned using these unsupervised methods, as recent research~\citep{shah2020pitfalls, geirhos2020shortcut} has pointed out
  that SL methods are vulnerable to spurious correlations: under certain settings, they learn \emph{only} features that are irrelevant to
  the true labelling functions yet highly predictive of the labels.
  %
  This leads to poor performance on \gls{OOD} test sets where the
  spurious features learned by the model are no longer present.
  %
  However, this behaviour is not surprising given SL's
  \emph{target-driven} objective (e.g. cross-entropy loss): when
  presented with two features that are equally predictive of the
  label, SL models have no incentive to learn both if learning only
  one of them suffices to accurately predict the target;
  %
  the choice then comes down to the inductive bias or the preference
  of the optimiser and the model architecture.
  % this could result in poor generalisation performance if the OOD test set relies on the overlooked feature.
  %
  Unsupervised learning objectives are, in comparison, more
  \emph{input-driven}, i.e. they learn to  maximise the mutual
  information between representations and the input data
  \citep{chen2020simclr,vib}.
  %
  We hypothesise that this characteristic behaviour of unsupervised
  objectives gives them a better chance to avoid the exploitation of
  spurious correlation, and thus faring better under distribution
  shift compared to supervised learning.
  
  \emph{\textbf{Contribution}: Systematically evaluate SSL and AE on distribution shift tasks.} We evaluate and compare the generalisation performance of unsupervised methods, including \gls{SSL} and \gls{AE}, with standard supervised learning. See \cref{sec:setup} for more details on our experiments.
  
  \vspace{-8pt}
  %
  \paragraph{Problem 2: Disconnect between synthetic and realistic datasets}
  %
  Broadly speaking, there exists two types of datasets for studying distribution
  shift: synthetic datasets where the shift between train/test
  distribution is explicit and controlled (e.g. MNIST-CIFAR
  \citep{shah2020pitfalls}, CdSprites \citep{fish}) and realistic
  datasets featuring distribution shift in the real world (e.g. WILDS
  \citep{koh2021wilds}). 
  %
  We provide visual examples in \cref{fig:synthetic_v_real}.
  %
  % However, even though both types of dataset sets out to study OOD generalisation, their usage are commonly seen in two different sub-fields: typically, works that discuss simplicity bias, dataset bias and shortcut learning focus on synthetic datasets \citep{teney2022evading, shah2020pitfalls, ahn2022mitigating}, while those that propose new domain generalisation/adaptation algorithms emphasise evaluating their model on realistic datasets \citep{sun2016coral, ganin2016dann}.
  
  Synthetic datasets allow for explicit control of the distribution
  shift and are, thus, an effective diagnostic tool for generalisation
  performance. However, the simplistic nature of these datasets poses
  concerns about the generality of the findings drawn from these
  experiments:
  %
  a model's robustness to spurious correlation on certain toy datasets
  is not very useful if it fails when tested on similar real-world
  problems.
  %
  On the other hand, realistic datasets often feature distribution
  shifts that are subtle, hard to define, and inconsistent across
  tasks~(see \cref{fig:synthetic_v_real}, right).
  %
  As a result, the generalisation performances tend to fluctuate
  across datasets~\citep{koh2021wilds, domainbed}, while the cause of
  such fluctuations remains unknown.
  
  % however we cannot explain what caused the change in results.
  
  \begin{figure*}[t]
      \centering
      \includegraphics[trim={0.5cm 0 0 0},clip, width=\linewidth]{images/hook.png}
      \vspace{-2em}
      \caption{\textbf{Synthetic vs. realistic distribution shift:} The distribution shift in synthetic datasets (\textit{left}, MNIST-CIFAR and CdSprites) are usually extreme and controllable (adjusted via changing the correlation); for realistic datasets (\textit{right}, WILDS-Camelyon17 and FMoW) distribution shift can be subtle, hard to identify and impossible to control.}
      % \vspace{-20pt}
      \label{fig:synthetic_v_real}
  \end{figure*}
  
  \emph{\textbf{Contribution}: Controllable but realistic distribution shift tasks.} In addition to evaluating models on both synthetic and
  realistic datasets, we subsample realistic domain generalisation datasets in WILDS to artificially create explicit correlation between domains and labels. 
  %
  This allows us to directly control the level of shift in these realistic distribution shift scenarios.
  %
  We refer to them as \emph{Controllable-Shift~(CS) datasets}.
  %
%   The resulting datasets utilise both real-world data and has
%   distribution shift that is controllable via the correlation
%   coefficient between domain and label information.
  %
  Note that there are datasets such as ImageNet-9, SVSF, or Waterbirds
  that provide distribution shift controls for real images, however
  our sub-sampling of realistic domain generalisation datasets allow
  us to gain such control cheaply, and in
  addition provide further analysis on models' performance on
  existing benchmarks (WILDS).
  
  \vspace{-8pt}
  \paragraph{Problem 3: The strong bias of linear classifier head}
  \citet{kang2019decoupling, menon2020overparameterisation} observed
  the interesting phenomenon that the final layer linear classifier in
  deep learning models is very susceptible to spurious
  correlation, and therefore a strong source of model bias. They
  showed that by simply retraining the linear classifier on data
  where the spurious correlation is absent, a model's performance on
  OOD test set can be dramatically improved.
  %
  This indicates that the representations, learned by the backbone of
  the model, are able to faithfully capture different features
  available in the input data. However, the linear classifier only
  assigns weights to some of those features (usually the simpler
  ones); and in many cases~\citep{shah2020pitfalls,kang2019decoupling}
  they appear to be spuriously correlated to the labels.
  %
  While previous investigations of this effect focused mainly on
  synthetic data, retraining the linear classifier head on OOD real
  world data can also potentially improve the performance on real
  distribution shift problems.
  % \footnote{This is similar to linear probing in transfer learning setting.}.
  %
  Importantly, if our interest lies in examining how well the
  \emph{representations} learned from different objectives capture
  available features in the data (and thereby generalise better to
  shifted distributions), we should aim to isolate the bias of the
  linear classification head by retraining it on data drawn from the
  same distribution as the OOD test set.
  
  \emph{\textbf{Contribution}: OOD linear head.} We report the
  OOD accuracy using a linear head trained on small amount of left-out
  \gls{OOD} data.
  %
  We also quantify the linear head bias to highlight the importance of this treatment when evaluating generalisation performance. 
  % More details in \cref{sec:setup}.
  
   
  
  In summary, we develop a suite of experiments and datasets to
  evaluate the performance of various learning paradigms under
  distribution shift.~\Cref{fig:summary} provides a summary of our
  results, comparing a wide range of algorithms from the following
  classes of objectives:
  %
  \begin{enumerate*}[label=(\roman*)]
  \item \gls{SSL},
  \item \gls{AE}, and 
  \item \gls{SL}.
  \end{enumerate*}
  %
  To the best of our knowledge, we are the first to systematically
  evaluate the performance of these different types of learning
  algorithms under distribution shift.
  %
  The models are evaluated on both synthetic and realistic
  distribution shift datasets, as well as shift-controlled realistic
  datasets that manufacture controllable, explicit spurious
  correlations.
  %
  The main takeaways from this paper are:
  
  
  %
  \begin{itemize}[nosep,leftmargin=1em,labelwidth=*,align=left]
     \item \textbf{SSL and AE are more robust than SL to extreme
     distribution shift:}
     \cref{fig:ms_summary,fig:cdsprites_summary,fig:camelyon_c_summary,fig:fmow_c_summary}
     shows results on distribution shift
     scenarios where the training set
     encodes extreme spurious correlations. For both synthetic
     (\Cref{fig:ms_summary,fig:cdsprites_summary}) and real world
     (\Cref{fig:camelyon_c_summary,fig:fmow_c_summary}) datasets, SSL
     and AE consistently outperforms SL in terms of OOD accuracy (top
     row); 
     \item \textbf{SSL and AE's performance is less sensitive to
     distribution shift than SL}: The bottom row of~\Cref{fig:summary}
     compares the shift sensitivity $s$ of different models 
     (see \cref{sec:setup} for definition). Smaller
     $s$ is desirable as it indicates lower sensitivity to
     distribution shift. Results show that SSL and AE algorithms are
     significantly more stable under distribution shift than SL;
    %  \item \textbf{SSL and AE's performance is less sensitive to
    %  distribution shift than SL}: The bottom row of~\Cref{fig:summary}
    %  shows the difference between ID and OOD accuracy (i.e. shift
    %  sensitivity $s$; see \cref{sec:setup} for definition). Smaller
    %  $s$ is desirable as it indicates lower sensitivity to
    %  distribution shift. Results show that SSL and AE algorithms are
    %  significantly more stable under distribution shift  than SL;
     \item \textbf{Generalisation performance on realistic
     distribution shift task can be significantly improved by
     retraining the last linear layer:} We show a large performance
     boost for all models, when evaluating using linear head trained
     on a small amount of OOD data, in contrast to the baseline where
     the linear head is trained on ID data. The surprising gain of
     this cheap procedure, even on realistic distribution shift
     problems, highlights the importance of isolating the linear head
     bias when evaluating models' generalisation performance.
  \end{itemize}

==> 2backgrounds_v5.tex <==

\begin{figure*}[t]
    \centering
    \captionsetup[subfigure]{belowskip=1ex}
    \begin{minipage}{\linewidth}
        \centering
        OOD Accuracy (higher is better)
    \end{minipage}
    \begin{subfigure}[t]{0.16\linewidth}
      \centering
      \includegraphics[width=\linewidth]{images/intro_plot/ms_acc.pdf}
    \end{subfigure}
    \begin{subfigure}[t]{0.16\linewidth}
      \centering
      \includegraphics[width=\linewidth]{images/intro_plot/cdsprites_summary_ood_shape.pdf}
    \end{subfigure}
    \begin{subfigure}[t]{0.16\linewidth}
      \centering
      \includegraphics[width=\linewidth]{images/intro_plot/camelyon17_corr100_acc.pdf}
    \end{subfigure}   
    \begin{subfigure}[t]{0.16\linewidth}
      \centering
      \includegraphics[width=\linewidth]{images/intro_plot/fmow_corr100_acc.pdf}
    \end{subfigure}  
    \begin{subfigure}[t]{0.16\linewidth}
      \centering
      \includegraphics[width=\linewidth]{images/intro_plot/camelyon17_corr0_acc.pdf}
    \end{subfigure}
    \begin{subfigure}[t]{0.16\linewidth}
      \centering
      \includegraphics[width=\linewidth]{images/intro_plot/fmow_corr0_acc.pdf}
    \end{subfigure} 
    \begin{minipage}{\linewidth}
        \centering
        OOD Error - ID Error (lower is better)
    \end{minipage}  
    \begin{subfigure}[t]{0.15\linewidth}
      \centering
      \includegraphics[width=\linewidth]{images/intro_plot/ms_rho.pdf}
      \caption{\scriptsize MNIST-CIFAR} \label{fig:ms_summary}
    \end{subfigure}
    \begin{subfigure}[t]{0.15\linewidth}
      \centering
      \includegraphics[width=\linewidth]{images/intro_plot/cdsprites_summary_rho.pdf}
      \caption{\scriptsize \centering CdSprites ($r_{\text{id}}=1$)}\label{fig:cdsprites_summary}
    \end{subfigure}
    \begin{subfigure}[t]{0.18\linewidth}
      \centering
      \includegraphics[width=0.838\linewidth]{images/intro_plot/camelyon17_corr100_rho.pdf}
      \caption{\scriptsize \centering Camelyon17-CS ($r_{\text{id}}=1$)}
      \label{fig:camelyon_c_summary}
    \end{subfigure}   
    \begin{subfigure}[t]{0.15\linewidth}
      \centering
      \includegraphics[width=\linewidth]{images/intro_plot/fmow_corr100_rho.pdf}
      \caption{\scriptsize \centering FMoW-CS ($r_{\text{id}}=1$)}\label{fig:fmow_c_summary}
    \end{subfigure}  
    \begin{subfigure}[t]{0.15\linewidth}
      \centering
      \includegraphics[width=\linewidth]{images/intro_plot/camelyon17_corr0_rho.pdf}
      \caption{\scriptsize Camelyon17}\label{fig:camelyon_summary}
    \end{subfigure}
    \begin{subfigure}[t]{0.15\linewidth}
      \centering
      \includegraphics[width=\linewidth]{images/intro_plot/fmow_corr0_rho.pdf}
      \caption{\scriptsize FMoW}\label{fig:fmow_summary}
    \end{subfigure} 
    
    \vspace{-1em}
    \caption{Performance of auto-encoder based (AE), \acrfull{SSL}, \acrfull{SL} models. \textbf{\textit{Top row}}: the OOD test set accuracy (\%) using linear heads trained on OOD data; \textbf{\textit{Bottom row}}: the difference in error rate  (\%) between evaluation on OOD test set vs. ID test set.}
    \label{fig:summary}
    \vspace{-12pt}
  \end{figure*}
  
  \subsection{Existing problems and Contributions} \label{sec:background}
  % \begin{itemize}[itemsep=1em,leftmargin=1em,labelwidth=*,align=left]
  % \vspace{-8pt}
  \paragraph{Problem 1: The outdated focus on supervised regime for distribution shift}
  %
  In ML research, distribution shfit is studied under varied
  terminologies such as simplicity bias~\citep{shah2020pitfalls},
  dataset bias~\citep{torralba2011datasetbias1}, shortcut
  learning~\citep{geirhos2020shortcut}, and domain adaptation and
  generalisation \citep{koh2021wilds, domainbed}.
  %
  However, most of them are done in the regime of supervised learning
  (SL), including various works that either investigate
  spurious correlations~\citep{shah2020pitfalls, hermann2020shapes,
  kalimeris2019sgd} or those that propose specialised methods to
  improve generalisation and/or avoid shortcut solutions~\citep{arjovsky2019irm, ganin2016dann, Sagawa2020dro,
  teney2022evading}.
  
  On the other hand, recent work in representation learning of images has seen a surge of unsupervised learning algorithms such as \acrfull{SSL}~(e.g., \citet{chen2020simclr,grill2020byol,chen2021simsiam}), which learn representations by enforcing invariance between the representations of two distinctly augmented views of the same image,  and \acrfull{AE}~\citet{rumelhart1985ae,kingma2013vae,higgins2016betavae,burda2015iwae}, which learn by reconstructing the input image.
  % such as \acrfull{SSL} and \acrfull{AE} \citep{chen2020simclr, grill2020byol, kingma2013vae, bao2021beit, he2021mae}.
  %
  While their impressive performance on various tasks led to their
  popularisation, these methods are mostly known for their
  strong performance on balanced \gls{ID} test datasets --- how they
  perform on distribution shift tasks remains largely unknown. 
  %
  We believe it is particularly meaningful to study the \acrfull{OOD}
  generalisation performance of the representations learned using these unsupervised methods, as recent research~\citep{shah2020pitfalls, geirhos2020shortcut} highlighted the extreme vulnerability of SL methods to spurious correlations: they are susceptible to learning \emph{only} features that are irrelevant to the true labelling functions yet highly predictive of the labels.
  %
  This leads to poor performance on \gls{OOD} test sets where the
  spurious features learned by the model are no longer present.
  %
  However, this behaviour is not surprising given SL's
  \emph{target-driven} objective (e.g. cross-entropy loss): when
  presented with two features that are equally predictive of the
  label, SL models have no incentive to learn both if learning only
  one of them suffices to accurately predict the target;
  %
  the choice then comes down to the inductive bias or the preference
  of the optimiser and the model architecture.
  % this could result in poor generalisation performance if the OOD test set relies on the overlooked feature.
  %
  Unsupervised learning objectives are, in comparison, more
  \emph{input-driven}, i.e. they learn to  maximise the mutual
  information between representations and the input data
  \citep{chen2020simclr,vib}.
  %
  We hypothesise that this characteristic behaviour of unsupervised
  objectives gives them a better chance to avoid the exploitation of
  spurious correlation, and thus faring better under distribution
  shift compared to supervised learning.
  
  \emph{\textbf{Contribution}: Systematically evaluate SSL and AE on distribution shift tasks.} We evaluate and compare the generalisation performance of unsupervised methods, including \gls{SSL} and \gls{AE}, with standard supervised learning. See \cref{sec:setup} for more details on our experiments.
  
  \vspace{-8pt}
  %
  \paragraph{Problem 2: Disconnect between synthetic and realistic datasets}
  %
  Broadly speaking, there exists two types of datasets for studying distribution
  shift: synthetic datasets where the shift between train/test
  distribution is explicit and controlled (e.g. MNIST-CIFAR
  \citep{shah2020pitfalls}, CdSprites \citep{fish}) and realistic
  datasets featuring distribution shift in the real world (e.g. WILDS
  \citep{koh2021wilds}). 
  %
  We provide visual examples in \cref{fig:synthetic_v_real}.
  %
  % However, even though both types of dataset sets out to study OOD generalisation, their usage are commonly seen in two different sub-fields: typically, works that discuss simplicity bias, dataset bias and shortcut learning focus on synthetic datasets \citep{teney2022evading, shah2020pitfalls, ahn2022mitigating}, while those that propose new domain generalisation/adaptation algorithms emphasise evaluating their model on realistic datasets \citep{sun2016coral, ganin2016dann}.
  
  Synthetic datasets allow for explicit control of the distribution
  shift and are, thus, an effective diagnostic tool for generalisation
  performance. However, the simplistic nature of these datasets poses
  concerns about the generality of the findings drawn from these
  experiments:
  %
  a model's robustness to spurious correlation on certain toy datasets
  is not very useful if it fails when tested on similar real-world
  problems.
  %
  On the other hand, realistic datasets often feature distribution
  shifts that are subtle, hard to define, and inconsistent across
  tasks~(see \cref{fig:synthetic_v_real}, right).
  %
  As a result, the generalisation performances tend to fluctuate
  across datasets~\citep{koh2021wilds, domainbed}, while the cause of
  such fluctuations remains unknown.
  
  % however we cannot explain what caused the change in results.
  
  \begin{figure*}[t]
      \centering
      \includegraphics[trim={0.5cm 0 0 0},clip, width=0.8\linewidth]{images/hook.png}
      \vspace{-1em}
      \caption{\textbf{Synthetic vs. realistic distribution shift:} The distribution shift in synthetic datasets (\textit{left}, MNIST-CIFAR and CdSprites) are usually extreme and controllable (adjusted via changing the correlation); for realistic datasets (\textit{right}, WILDS-Camelyon17 and FMoW) distribution shift can be subtle, hard to identify and impossible to control.}
       \vspace{-20pt}
      \label{fig:synthetic_v_real}
  \end{figure*}
  
  
  \emph{\textbf{Contribution}: Controllable but realistic distribution shift tasks.} In addition to evaluating models on both synthetic and
  realistic datasets, we subsample realistic domain generalisation datasets in WILDS to artificially create explicit correlation between domains and labels. 
  %
  This allows us to directly control the level of shift in these realistic distribution shift scenarios.
  %
  We refer to them as \emph{Controllable-Shift~(CS) datasets}.
  %
%   The resulting datasets utilise both real-world data and has
%   distribution shift that is controllable via the correlation
%   coefficient between domain and label information.
  %
  Note that there are datasets such as ImageNet-9, SVSF, or Waterbirds
  that provide distribution shift controls for real images, however
  our sub-sampling of realistic domain generalisation datasets allow
  us to gain such control cheaply, and in
  addition provide further analysis on models' performance on
  existing benchmarks (WILDS).
  
  \vspace{-8pt}
  \paragraph{Problem 3: The strong bias of linear classifier head}
  The most popular evaluation protocol for representation learning algorithms (both supervised and unsupervised) is \emph{linear probing}, which trains a linear classifier head on top of the representation learning model with frozen weights to predict the labels.
  %
  \citet{kang2019decoupling, menon2020overparameterisation} observed
  the interesting phenomenon that the final layer linear classifier can be extremely susceptible to spurious
  correlation, causing poor OOD performance: under simple, synthetic set up, they showed that SL models' performance on OOD test set can be dramatically improved by simply retraining the linear classifier on data where the spurious correlation is absent.
  %
  This indicates that the linear classifier can be a strong source of model bias in distribution shift tasks --- if one's interests lies in examining the robustness of representations/backbone model, it is important to isolate this bias by re-training the linear head on OOD data during evaluation.
  %
  To the best of our knowledge, while this finding is well-established in long-tailed recognition and simplicity bias problems, retraining linear head on OOD data is not yet standard evaluation protocol in areas such as domain generalisation.
  %while the representations learned by the backbone model can able to faithfully capture different features
%   available in the input data, the linear classifier only
%   assigns weights to some of those features (usually the simpler
%   ones); and in many cases~\citep{shah2020pitfalls,kang2019decoupling}
%   they appear to be spuriously correlated to the labels.
  %
%   While previous investigations of this effect focused mainly on
%   synthetic data and SL algorithms, we investigate whether 
%   retraining the linear classifier head on OOD real world data can also potentially improve the performance on real
%   distribution shift problems.
  
  \emph{\textbf{Contribution}: OOD linear head.} We introduce the OOD linear head evaluation as a standard protocol for evaluating robustness of representation learning algorithms to distribution shift. This allows for isolating the bias of the linear classification head by reporting the OOD accuracy using a linear head trained on small amount of left-out \gls{OOD} data.
  %
  We also quantify the linear head bias to highlight the importance of this treatment when evaluating generalisation performance. 
  % More details in \cref{sec:setup}.
  
   
  
  In summary, we develop a suite of experiments and datasets to
  evaluate the performance of various learning paradigms under
  distribution shift.~\Cref{fig:summary} provides a summary of our
  results, comparing a wide range of algorithms from the following
  classes of objectives:
  %
  \begin{enumerate*}[label=(\roman*)]
  \item \gls{SSL},
  \item \gls{AE}, and 
  \item \gls{SL}.
  \end{enumerate*}
  %
  To the best of our knowledge, we are the first to systematically
  evaluate the performance of these different types of learning
  algorithms under distribution shift.
  %
  The models are evaluated on both synthetic and realistic
  distribution shift datasets, as well as shift-controlled realistic
  datasets that manufacture controllable, explicit spurious
  correlations.
  %
  The main takeaways from this paper are:
  
  
  %
  \begin{itemize}[nosep,leftmargin=1em,labelwidth=*,align=left]
     \item \textbf{SSL and AE are more robust than SL to extreme
     distribution shift:}
     \cref{fig:ms_summary,fig:cdsprites_summary,fig:camelyon_c_summary,fig:fmow_c_summary}
     shows results on distribution shift
     scenarios where the training set
     encodes extreme spurious correlations. For both synthetic
     (\Cref{fig:ms_summary,fig:cdsprites_summary}) and real world
     (\Cref{fig:camelyon_c_summary,fig:fmow_c_summary}) datasets, SSL
     and AE consistently outperforms SL in terms of OOD accuracy (top
     row); 
     \item \textbf{SSL and AE's performance is less sensitive to
     distribution shift than SL}: The bottom row of~\Cref{fig:summary}
     compares the shift sensitivity $s$ of different models 
     (see \cref{sec:setup} for definition). Smaller
     $s$ is desirable as it indicates lower sensitivity to
     distribution shift. Results show that SSL and AE algorithms are
     significantly more stable under distribution shift than SL;
    %  \item \textbf{SSL and AE's performance is less sensitive to
    %  distribution shift than SL}: The bottom row of~\Cref{fig:summary}
    %  shows the difference between ID and OOD accuracy (i.e. shift
    %  sensitivity $s$; see \cref{sec:setup} for definition). Smaller
    %  $s$ is desirable as it indicates lower sensitivity to
    %  distribution shift. Results show that SSL and AE algorithms are
    %  significantly more stable under distribution shift  than SL;
     \item \textbf{Generalisation performance on realistic
     distribution shift task can be significantly improved by
     retraining the last linear layer:} We show a large performance
     boost for all models, when evaluating using linear head trained
     on a small amount of OOD data, in contrast to the baseline where
     the linear head is trained on ID data. The surprising gain of
     this cheap procedure, even on realistic distribution shift
     problems, highlights the importance of isolating the linear head
     bias when evaluating models' generalisation performance.
  \end{itemize}

==> 3methods_v1.tex <==
\section{Set-up} \label{sec:setup}

In \cref{sec:introduction} we identified three problems within our existing field.
%
In this section, we will introduce the experimental set-up we used to address them in further details.

\textbf{Algorithms:} \emph{$\times$3 SSL, $\times$4 AE, $\times$1 SL.}
%
For all experiments we report results on seven types of learning algorithms, including three \gls{SSL} algorithms 1) SimCLR \citep{chen2020simclr}, 2) SimSiam \citep{chen2021simsiam}, 3) BYOL \citep{grill2020byol}; four \gls{AE} algorithms 1) Autoencoder \citep{rumelhart1985ae}, 2) \gls{VAE} \citep{kingma2013vae}, 3) $\beta$-\gls{VAE} \citep{higgins2016betavae} and 4) \gls{IWAE} \citep{burda2015iwae}.
%
These popular methods in \gls{SSL} and latent generative models have not yet been systematically evaluated under distribution shift tasks.
%
We compare the performance of these models against standard supervised learning (SL).

\textbf{Datasets:} \emph{$\times$2 synthetic, $\times$2 realistic, $\times$2 controllable realistic.}
%
We evaluate our models on two synthetic datasets, namely MNIST-CIFAR \citep{shah2020pitfalls} (\Cref{subsec:mnist_cifar}) and CdSprites \citep{fish} (\Cref{subsec:cdsprites_experiment}), as well as two realistic datasets from WILDS \citep{koh2021wilds}, including Camelyon17 and FMoW (\Cref{sec:wilds_original}).
%
To further understand models' performance and draw conclusions that are meaningful to scenarios beyond the ones that we studied, we also subsample the training set of Camelyon17 and FMoW datasets to create spurious correlation between the domain and label information.
%
Changing this correlation varies the degree of distribution shift between train and test split, which allows us to analyse models' performance more effectively under realistic distribution shift settings.
%
We refer to this controllable version of the two datasets Camelyon17-C and FMoW-C, and provide further details on the datasets in \cref{sec:wilds_controllable}.



\textbf{Evaluation:} \emph{3 metrics.}
%
For convenience of discussion, let us define some notations first. 
%
We write the backbone model (excluding linear head) trained on ID train set as $f$, the linear head trained on ID train set as $c_i$, and trained on OOD test set as $c_o$;
%
further, we denote the accuracy of a backbone model $f$ and linear head $c$ on ID test data as acc$_i(f,c)$, and on OOD test data as acc$_o(f,c)$.

\citet{kang2019decoupling, menon2020overparameterisation, kirichenko2022last} discover that the linear classifier $c$ is a surprisingly significant source of model's bias: they find that by simply retraining the linear head on de-biased (OOD) data, the model's performance on OOD data can be drastically improved.
%
Since our interests lie in evaluating the representations learned by the backbone models, we report our results using linear head trained on OOD data, i.e. \aoco.
%
Additionally, to quantify the bias introduced by the linear head trained on ID data, we define the \emph{linear head bias} as the difference between the OOD accuracy evaluated by OOD linear head and ID linear head, i.e.
\begin{align}
    b = \aoco - \aoci. \label{eq:b}
\end{align}


In addition, we measure the \emph{effective robustness} of the model $f$ (initially proposed by \citet{taori2020measuring}) to disentangle a model's generalisation performance from its performance on standard (ID) test set.
%
The effective robustness can be computed as
%
\begin{align}
    \rho = \aoco - \aici. \label{eq:rho}
\end{align}
%
A large $\rho$ is desirable, as it indicates that the performance of the model does not drop much with distribution shift on the test set.
%
Note that our version differs from \citet{taori2020measuring}: we omit the baseline accuracy parameter $\beta$; in addition, the original version does not utilise $c_o$ and they compute instead $\aoci-\aici$. 
%
In contrast, our version evaluates the effective robustness without the impact of the linear head bias.

In summary, for each experiment we report the following three metrics: OOD linear head accuracy $\aoco$, linear head bias $b$ and effective robustness $\rho$.

==> 3methods_v2.tex <==
\section{Set Up} \label{sec:setup}

In \cref{sec:introduction} we identified three problems in the
existing literature that we wish to address in this work.
%
In this section, we will introduce the necessary experimental set-up
to address them in further details. In brief, we compare seven ML
algorithms on six datasets using three relevant metrics.

\textbf{Algorithms:} \emph{$\times$3 SSL, $\times$4 AE, $\times$1 SL.}
%
For all our experiments, we compare seven representation learning
algorithms, including three \gls{SSL} algorithms 1) SimCLR
\citep{chen2020simclr}, 2) SimSiam \citep{chen2021simsiam}, and 3)
BYOL \citep{grill2020byol}; and four \gls{AE} algorithms 1)
Autoencoder \citep{rumelhart1985ae}, 2) \gls{VAE}
\citep{kingma2013vae}, 3) $\beta$-\gls{VAE} \citep{higgins2016betavae}
and 4) \gls{IWAE} \citep{burda2015iwae}.
%
These popular methods in \gls{SSL} and latent generative models have
not yet been systematically evaluated under distribution shift tasks
prior to our work.
%
We compare the performance of these models against a standard
supervised learning (SL) algorithm used as a representation learning
model.

\textbf{Datasets:} \emph{$\times$2 synthetic, $\times$2 realistic,
$\times$2 controllable shift.}
%
We evaluate our models on two synthetic datasets, namely MNIST-CIFAR~(\citet{shah2020pitfalls}; see \cref{subsec:mnist_cifar}) and CdSprites~(\citet{fish}; see~\Cref{subsec:cdsprites_experiment}), as well as two
realistic datasets from WILDS~\citep{koh2021wilds}:
Camelyon17 and FMoW (see~\Cref{sec:wilds_original}).
%
However, as mentioned in~\Cref{sec:background}, both the synthetic and
the realistic datasets have their own drawbacks. To further
understand the models' performance and draw conclusions that are
generalisable, we also provide a framework
for creating {\em controllable shift} datasets from realistic datasets
like those in WILDS, by subsampling the data to introduce spurious correlations between the domain and label information in the training set.
%
Changing this correlation varies the degree of distribution shift
between the~(ID) train and~(OOD) test split, which allows us to
analyse the models' performance more effectively under realistic, yet
controllable, distribution shift.
%
We refer to this controllable shift versions of the two datasets
Camelyon17-CS and FMoW-CS, and provide further details on the datasets
in~\Cref{sec:wilds_controllable}.



\textbf{Evaluation:} \emph{3 metrics.}
%
% We use three metrics to understand various facets of this problem.
For convenience of discussing our proposed metrics, we will first define some notations. 
%
We separate a model trained to perform a particular task into two parts, namely, 1) backbone $f$, denoting the part of the model that generates representations from the data, and 2) final linear head $c$, which takes the representations from $f$ and outputs the final prediction.
%
Further, we refer to the final linear head trained on the ID train set as $c_i$, and that trained on the OOD test set as $c_o$.
%
Note that since the backbone model $f$ is always trained on the ID train set, we do not make any special distinction on its training distribution. 
%
We also denote the accuracy of $f$ and $c$ on the ID test data as
acc$_i(f,c)$, and on the OOD test data is referred to as acc$_o(f,c)$.

\citet{kang2019decoupling, menon2020overparameterisation} discovered
that the linear classifier $c$ is a surprisingly significant source of
bias in the model. Their experiments showed that simply retraining the linear head, on de-biased (OOD) data, drastically improves the
model's performance on OOD data.
%
Since our interests lie in evaluating the representations learned by
the backbone models, we report our results using linear head trained
on OOD data, i.e. \aoco~ in order to disentangle the bias of the linear
head.
%
To quantify this bias introduced by training the linear head on ID
data, we measure the difference between the OOD test accuracy
evaluated by OOD linear head and the OOD accuracy evaluated by the ID
linear head, and refer to it as \emph{linear head bias}:
\begin{align}
    b = \aoco - \aoci. \label{eq:b}
\end{align}


In a related work,~\citet{taori2020measuring} argued about the
necessity to disentangle a model's generalisation performance from its
standard (ID) test accuracy. Instead of measuring the ID test
accuracy, they proposed to measure the \emph{effective robustness} of
the model as $\rho = \aici - \aoci$. 
%
A small $\rho$ is desirable, as it indicates that the performance of
the model is relatively insensitive to a distribution shift on the
test set\footnote{We negate the original definition of effective
robustness from~\citet{taori2020measuring} for ease of
understanding.}.
%
However, we note that a simple decomposition of \emph{effective
robustness}~(\(\rho\)) shows a hidden {\em linear head bias}~(\(b\))
term
\vspace{3pt}
\begin{align}
    \underbrace{\aici - \aoci}_{\text{effective robustness}~\rho} &= \aici - \aoci  - \aoco + \aoco \notag \\
    &= \underbrace{\aici - \aoco}_{\text{linear head bias}~b} + \underbrace{\aoco - \aoci}_{\text{shift sensitivity}~s}. \label{eq:s}
\end{align}
%
Since we are primarily interested in the robustness of the
representations of the backbone model $f$, and not the classifier head
$c$, we need to remove the effect of the linear head bias from the
effective robustness. Thus, we  report the last term in \Cref{eq:s},
which we name {\em shift sensitivity}, denote as $s=\rho- b$.
%
Alternatively, it is the difference between the OOD accuracy using
linear head trained on OOD data, and ID accuracy using linear head
trained on ID data.
%
Larger $s$ marks higher sensitivity of $f$ to distribution shift,
which is, possibly, dangerous for the deployment of such models.

In summary, for each experiment we report the following three metrics: OOD linear head accuracy $\aoco$, linear head bias $b$ and shift sensitivity $s$.

==> 4experiments_v1.tex <==


\section{Experimental results} \label{sec:experiments}




\begin{table}[t]
\centering
\caption{Evaluations on OOD test set of MNIST-CIFAR dataset. We report accuracy on MNIST and CIFAR trained using OOD linear head ($\text{acc}_o(f,c_o)$), linear head bias ($b$) and effective robustness ($\rho$).}
\vspace*{-0.8\baselineskip}
\scalebox{0.78}{
\begin{tabular}{llccccccc}    \toprule
    \multirow{2}{*}{Regime} &\multirow{2}{*}{Method} & \multicolumn{3}{c}{MNIST (\%)} & & \multicolumn{3}{c}{CIFAR (\%)}  \\
    \cmidrule{3-5} \cmidrule{7-9}
    & &  $\text{acc}_o(f,c_o)\uparrow$ & $\rho \downarrow$ & $b$ && $\text{acc}_o(f,c_o)\uparrow$ & $\rho\downarrow$  & $b$ \\
    \midrule \rowcolor{lb}
    & AE  & 99.9 \std{1e-2} & 0.0 \std{1e-2} & 0.4 \std{2e-3} && 81.1 \std{1e+0} & 18.8 \std{1e+0} & 30.2 \std{1e+0}\\  \rowcolor{lb}
    & VAE  & 99.8 \std{8e-3} & -0.1 \std{9e-3} & 1.5 \std{1e-4} && 79.7 \std{4e+0} & 20.2  \std{3e+0} & 29.2  \std{6e+0}\\  \rowcolor{lb}
    & IWAE  & 99.8 \std{9e-3} & 0.0 \std{4e-3} & 1.4 \std{5e-3} && 80.8 \std{2e+0} & 19.0 \std{3e+0} & 30.0  \std{4e+0}\\  \rowcolor{lb}
    \multirow{-4}{*}{AE}
    & $\beta$-VAE  & 99.8 \std{2e-2} & 0.0 \std{4e-2} & 1.7 \std{3e-2} && 78.0 \std{3e+0} & 21.8  \std{4e+0} & 28.0  \std{4e+0}\\  \rowcolor{db}
    \multicolumn{2}{l}{\emph{\textbf{AE average}}} & \emph{\textbf{99.8 \std{1e-2}}}  & \emph{0.0 \std{1e-2}}  & \emph{1.3 \std{9e-3}} && \emph{79.9 \std{3e+0}}  & \emph{20.0  \std{3e+0}} & \emph{29.3  \std{4e+0}} \\
    \midrule \rowcolor{lg}
    & SimCLR  & 99.7 \std{1e-2} & 0.2 \std{1e-3} & 0.2 \std{3e-3} && 85.8 \std{1e+0} & 14.1 \std{2e+0} & 35.5  \std{1e+0}\\ \rowcolor{lg}
    & SimSiam  & 99.8 \std{2e-1} & 0.1 \std{2e-1} & 1.6 \std{9e-2} && 87.8 \std{2e+0} & 12.1  \std{2e+0} & 35.6  \std{4e+0}\\  \rowcolor{lg}
    \multirow{-3}{*}{SSL} 
    & BYOL  & 99.8 \std{4e-2} & 0.0 \std{1e-2} & 0.9 \std{8e-3} && 84.8 \std{9e-1} & 15.0  \std{1e+0} & 33.2  \std{1e+0}\\  \rowcolor{dg}
    \multicolumn{2}{l}{\emph{\textbf{SSL average}}} & \emph{\textbf{99.8 \std{8e-2}}} & \emph{\textbf{0.1} \std{5e-2}} & \emph{1.2 \std{3e-2}} && \emph{\textbf{86.1 \std{1e+0}}} & \emph{\textbf{13.7 \std{2e+0}}} & \emph{34.8 \std{2e+0}} \\
    \midrule \rowcolor{g}
    SL
    & Supervised  & 97.7 \std{9e-1} & 1.4 \std{1e+0} & -0.3 \std{1e+0} && 51.5 \std{1e+0} & 47.6  \std{1e+0} & 0.8  \std{9e-1}\\ 
    \bottomrule
\end{tabular}
\label{tab:mnist_cifar_results}}
\vspace*{-\baselineskip}
\end{table}



%
We perform a hyperparameter search on learning rate, scheduler, optimiser, representation size, etc. for each model, and we use the same set of augmentations for all models to ensure a fair comparison.
%
See \cref{sec:app_hp} for more details.

\subsection{Synthetic distribution shift}  \label{sec:simplicity}
%
\textbf{\emph{Findings:}} \emph{With a perfect correlation between the complex and simple features in the data, representations learned by \gls{SSL} and \gls{AE} models capture both features, while \gls{SL} focusses on the simpler features only.}

We are interested in understanding whether models pre-trained with \gls{SL}, \gls{SSL} and \gls{AE} methods are vulnerable to simplicity bias under synthetic distribution shift settings.
%
Following \citet{shah2020pitfalls, fish}, we evaluate this using the MNIST-CIFAR and CdSprites datasets. 

\subsubsection{MNIST-CIFAR} \label{subsec:mnist_cifar}
%
Following \citet{shah2020pitfalls}, we use the MNIST-CIFAR dataset to examine the simplicity bias of different models. 
%

\begin{wrapfigure}[12]{r}{0.2\linewidth}
\vspace{-0.8em}
\begin{subfigure}{0.99\linewidth}
    \includegraphics[width=0.95\linewidth]{images/mnist_cifar/ms_id.png}
    \vspace{-4pt}
    \subcaption{ID}\label{fig:ms_id_vis}
\end{subfigure}\\
\begin{subfigure}{0.99\linewidth}
    \includegraphics[width=0.95\linewidth]{images/mnist_cifar/ms_ood.png}
    \vspace{-4pt}
    \subcaption{OOD}\label{fig:ms_ood_vis}
    % \vspace{-10pt}
\end{subfigure}
\caption{MNIST-CIFAR dataset.}\label{fig:ms}
\end{wrapfigure}
%
The dataset consists of concatenations of images from 2 classes of MNIST and CIFAR-10. 
%
It contains the following splits with varying correlation between the labels of the MNIST and CIFAR-10 images:

\begin{itemize}[nosep,leftmargin=1em,labelwidth=*,align=left]
    \item \textbf{ID train}: $1.0$ correlation between MNIST and CIFAR-10 labels. Contains two classes: class 0 with MNIST ``0'' and CIFAR-10 ``automobile'', and class 1 with MNIST ``1'' and CIFAR-10 ``plane'' (\Cref{fig:ms_id_vis});
    \item \textbf{OOD train}: no correlation between MNIST and CIFAR-10 labels, images from the two classes of MNIST and CIFAR-10 are randomly paired (\Cref{fig:ms_ood_vis});
    \item \textbf{OOD test}: generated similarly to the \gls{OOD} train set using the test set of MNIST and CIFAR-10 (\Cref{fig:ms_ood_vis}). 
\end{itemize}

% \setlength{\intextsep}{5pt}%
% \setlength{\columnsep}{8pt}%


We train a CNN backbone on the ID train set using the respective \gls{SL}, \gls{SSL}, or \gls{AE} algorithm. At test time, we freeze the backbone and train two linear heads, one on ID train and the other on OOD train, and evaluate their performance on the OOD test set.
%
This helps us disentangle the simplicity bias of the representation from that of the linear head.

% \looseness=-1
In \cref{fig:mnist_cifar,fig:ms_summary},
%
we observe that with \gls{ID} linear head, all models exhibit a simplicity bias, as the classifiers reach near $100\%$ accuracy for the classification of the MNIST digit (\Cref{fig:ms_mnist}, left) but near random accuracy for predicting the CIFAR class (\Cref{fig:ms_cifar}, left).
%
However, the \gls{OOD} linear head results indicate that both \gls{SSL} and \gls{AE} models are able to learn representations that capture \emph{both} features, with not only near perfect accuracy on MNIST (\Cref{fig:ms_mnist}, right), but also $\~80\%$ accuracy on CIFAR-10 (\Cref{fig:ms_cifar}, right).
%
On the other hand, representations learned using \gls{SL} do not extract~(linearly separable) CIFAR-10 features, since its OOD evaluation performance is near random on CIFAR-10.
%
%Another 

Interestingly, %observation from 
\Cref{fig:ms_summary} shows that using OOD linear head, the average performance of models trained using \gls{SSL} is $\~5$ percentage points higher than that of~\gls{AE}, while \gls{AE} scores $\~30$ percentage points higher than \gls{SL}.

\begin{figure*}[t]
  \centering
  \captionsetup[subfigure]{belowskip=1ex}
  \begin{subfigure}{0.44\linewidth}
    \centering
    \includegraphics[width=0.49\linewidth]{images/cdsprites/id_color_v.pdf}
    \includegraphics[width=0.49\linewidth]{images/cdsprites/ood_color_v.pdf}
    \caption{Color classification, OOD acc (\%).}\label{fig:cdsprites_color}
  \end{subfigure} \vspace{20pt}
  \begin{subfigure}{0.44\linewidth}
    \centering
    \includegraphics[width=0.49\linewidth]{images/cdsprites/id_shape_v.pdf}
    \includegraphics[width=0.49\linewidth]{images/cdsprites/ood_shape_v.pdf}
    \caption{Shape classification, OOD acc (\%).}\label{fig:cdsprites_shape}
  \end{subfigure}
  \vspace{-20pt}
  \caption{Evaluations on the CdSprites dataset. Blue colors are \gls{AE} models, green colors are \gls{SSL} models and grey is \gls{SL}. {\textbf{\Cref{fig:cdsprites_color}:}} Color classification accuracy on the test set with a linear head trained on ID data (left, transparent) and OOD data (right, solid); {\textbf{\Cref{fig:cdsprites_shape}:}} Shape classification accuracy on the \gls{OOD} test set with a linear head trained on ID data (left, transparent) and OOD data (right, solid).
  }
%   \vspace{-12pt}
  \label{fig:cdsprites_individual}
\end{figure*}

\subsubsection{CdSprites}  \label{subsec:cdsprites_experiment}
\looseness=-1
CdSprites \citep{fish} is a colored variant of the popular dSprites dataset \citep{dsprites}, which consists of images of 2D shapes that are procedurally generated from 6 ground truth factors (see \cref{fig:cdsprites_example} for examples). To induce a spurious correlation between the color and shape features, the sprites are colored conditionally on the shape and depending on the correlation coefficient $\rho$ that is set when generating the dataset. We generate five versions of the CdSprites dataset with a different correlation coefficient $\rho \in \{0, 0.25, 0.5, 0.75, 1.0\}$ respectively and use the following splits: 
\begin{itemize}[nosep,leftmargin=1em,labelwidth=*,align=left]
    \item \textbf{ID train}: CdSprites dataset with correlation $\rho_{\text{id}}$ between shape and color features; % used to train a CNN backbone with the respective \gls{SL}, \gls{SSL}, or \gls{AE} algorithm.
    \item \textbf{OOD train}: CdSprites dataset with uncorrelated shape and color features, i.e., $\rho_{\text{ood}}=0$; %used to train a linear head on top of the trained but frozen backbone.
    \item \textbf{OOD test}: generated similarly to the \gls{OOD} train set. % used to evaluate the linear head on holdout data.
\end{itemize}
%

\begin{wrapfigure}[12]{r}{0.3\linewidth}
     \centering
     \vspace{-1.5em}
     \begin{subfigure}[b]{0.45\linewidth}
         \centering
         \includegraphics[width=\linewidth]{images/cdsprites/cdsprites_example_corr0.png}
         \caption{$\rho = 0$}
         \label{subfig:cdsprites_example_corr0}
     \end{subfigure}
     \begin{subfigure}[b]{0.45\linewidth}
         \centering
         \includegraphics[width=\linewidth]{images/cdsprites/cdsprites_example_corr100.png}
         \caption{$\rho = 1$}
         \label{subfig:cdsprites_example_corr100}
     \end{subfigure}
     \caption{The CdSprites dataset. Each subplot shows 16 samples from the dataset generated with a given correlation~$\rho$ between shape and color features.}
     \label{fig:cdsprites_example}
     \vspace{1.0em}
\end{wrapfigure}

Based on the above splits, we use the same evaluation protocol as for MNIST-CIFAR (see \cref{subsec:mnist_cifar}) to disentangle the simplicity bias of the representation from the simplicity bias of the linear classification head.
% The above protocol allows us to test the performance of the different backbones in-distribution ($\rho_{\text{id}} = \rho_{\text{ood}}$) and out-of-distribution ($\rho_{\text{id}} \not= \rho_{\text{ood}}$), and to disentangle the simplicity bias of the representation from the simplicity bias of the linear classifier head.

% First, we train the backbones (i.e., the different algorithms from the classes of \gls{SL}, \gls{SSL}, and \gls{AE} methods) on CdSprites with spurious correlation $\rho_{\text{train}} \in \{0, 0.25, 0.5, 0.75, 1.0\}$. Then, we train the classifiers on the frozen representation from input data with $\rho_{\text{val}} = 0$. Finally, we test the classifiers on a holdout set with $\rho_{\text{test}} = 0$. This protocol allows us to test the performance of the different backbones in-distribution ($\rho_{\text{train}} = \rho_{\text{val}} = \rho_{\text{test}}$) and out-of-distribution ($\rho_{\text{train}} \not= \rho_{\text{val}} = \rho_{\text{test}}$).
% \jimmy{I think you need to specify more clearly (maybe with bullet points and visualisation of the dataset) that 1. train dataset (id): varying degree of correlation 2. test dataset (ood): 0 correlation between color and shape 3. val dataset (ood): 0 correlation between color and shape (used for ood evaluation)}. 

\Cref{fig:cdsprites_summary,fig:cdsprites_individual} show the results for backbones trained on data with a perfect correlation ($\rho_{\text{id}} = 1$) between shape and color features. Similar to MNIST-CIFAR, with the ID linear head we observe a simplicity bias, where the performance on the simple feature (color, \cref{fig:cdsprites_color}) is perfect and the performance on the complex feature (shape, \cref{fig:cdsprites_shape}) is trivial. Again, the OOD linear head results (right subplots of \cref{fig:cdsprites_color,fig:cdsprites_shape} respectively) indicate that \gls{AE} and especially \gls{SSL} models are able to learn representations that capture \emph{both} shape and color features.
% We observe that the representations from all \gls{SSL} and \gls{AE} models yield a high OOD classification accuracy, when we train an MLP classifier on top of the frozen representation. In comparison, supervised models show a significantly worse performance on OOD data.
We also provide results with changing values of \rhoid~and \rhoood\ in \Cref{app:cdsprites}.
% \cref{fig:cdsprites_corrx_ood0} shows the results for backbones trained on data with correlation $\rho_{\text{id}}$ and OOD linear heads trained and evaluated on data with uncorrelated data. Notably, with imperfect correlation ($\rho_{\text{id}} < 1$), the OOD linear heads trained on top of the \gls{SL} and \gls{SSL} backbones perform perfectly. For the \gls{AE}, we observe that the performance of the OOD linear head does not depend on the correlation $\rho_{\text{id}}$ in the data used to train the backbones. Our results suggest that with imperfect correlation between features, \gls{SL} and \gls{SSL} models learn a linearly separable representation of the features, whereas \gls{AE} does not. We provide additional results in \Cref{app:additional_results}.


%
% Notably, SSL and AE models are robust to spurious correlations $\rho_{\text{id}}$ of any degree and maintain high OOD classification accuracy on non-correlated data. In contrast, SL shows good OOD classification accuracy only when trained on data with spurious correlation $\rho_{\text{id}} < 1$.

% \imant{@Jimmy, Amartya: what do you think about the result described in the last paragraph? We might need to position it carefully with respect to the other results we have. Note that I did not yet run the evaluation on data with corr > $0$.}
% \jimmy{If I understood you correctly (see slack message), I think the evaluation you presented here is more important than evaluation on ID data, but for the sake of completeness it would be good to have the eval on ID data. I think the results are great, but maybe instead of phrasing it as "SSL/AE's advantage diminish as spurious corr. decrease", we swap the above two paragraph around and say something like: "SL does fine when no spurious correlation exist in the ID training data, however its performance heavily drops as spurious correlation increase, while  SSL and AE are able to avoid the pitfall of spurious correlation and maintain high test accuracy on non-correlated data. Specifically, when corr=0, SL, SSL and AE all has accuracy X, however when corr=1, SL's accuracy is X, while SSL and AE are X. This further demonstrates that <labels are BAD blah blah>"}


% \begin{figure}
%      \centering
%      \includegraphics[width=0.98\linewidth]{images/cdsprites/cdsprites_ood0.pdf}
%      \vspace{-1em}
%      \caption{Evaluations on CdSprites. Shape classification accuracy as a function of the correlation between shape and color features ($\rho_{\text{id}}$, x-axis) in the ID train split used to pre-train the respective backbone. Linear heads were trained on top of the frozen backbones using the OOD train split. Blue colors are AE models, green colors are SSL models, and grey is SL. The black horizontal line denotes the random baseline (33.3\% for three classes).}
%      \label{fig:cdsprites_corrx_ood0}
%      \vspace{-1.0em}
% \end{figure}
% \begin{figure}
%      \centering
%      \begin{subfigure}[b]{0.32\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{images/corr100_ood0.png}
%          \caption{Backbones trained on perfectly correlated data. Classifiers trained on top of the frozen representations from the respective backbone using uncorrelated data as input.}
%          \label{subfig:cdsprites_corr100_ood0}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{0.65\textwidth}
%          \centering
%          % \includegraphics[width=\textwidth]{images/corrx_oody.png}
%              \begin{subfigure}[b]{0.32\textwidth}
%                  \centering
%                  \includegraphics[width=\textwidth]{images/corrx_oody_ae.png}
%                  \caption*{AE}
%              \end{subfigure}
%              \begin{subfigure}[b]{0.32\textwidth}
%                  \centering
%                  \includegraphics[width=\textwidth]{images/corrx_oody_ssl.png}
%                  \caption*{SSL}
%              \end{subfigure}
%              \begin{subfigure}[b]{0.32\textwidth}
%                  \centering
%                  \includegraphics[width=\textwidth]{images/corrx_oody_sl.png}
%                  \caption*{SL}
%              \end{subfigure}
%          \caption{Backbones trained on data with spurious correlation=$x$. MLP classifiers trained (and tested) on top of the frozen representations from the respective backbone using spurious correlation=$y$.}
%          \label{subfig:cdsprites_corrx_oody}
%      \end{subfigure}
%      \caption{Results for the CdSprites experiment. \textit{Left:} OOD classification performance using perfectly correlated data to train the backbones. \textit{Right:} Varying the spurious correlation of the training data and OOD test data.}
% \end{figure}





\subsection{Real-world distribution shift}  \label{sec:dg} 
%
\textbf{\emph{Findings:}} \emph{Learning with labels (SL) is no better than learning without labels (SSL, AE) for \gls{OOD} generalisation on real-world distribution shift problems, and the performance of all models can be significantly improved by retraining the linear head on a small amount of OOD data.}

In this section we investigate the performance of different pre-trained models on real-world distribution shift tasks. 
%
We utilise the Camelyon17 dataset from the WILDS benchmark \citep{koh2021wilds}, which contains scans of lymph node sections acquired from different hospitals, and the task is to determine whether a given patch contains breast cancer tissue.
%
In addition to evaluating on the original dataset, we create a simplicity bias (SB) version of Camelyon17 (Camelyon17\_SB) by sub-sampling the ID train split of the Camelyon17 dataset such that the label and domain of each sample are perfectly correlated. This allows us to examine the OOD generalisation performance of different models on a more challenging but still realistic distribution shift task.

\subsection{Camelyon17} \label{sec:camelyon17}
\looseness=-1
The original Camelyon17 dataset from WILDS benchmark contains three splits using tissue scans from five hospitals: train (3 hospitals), validation (1 hospital) and test (1 hospital).
%
We further create four splits specified as follows:
%
\begin{itemize}[nosep,leftmargin=1em,labelwidth=*,align=left]
    \item \textbf{ID train}: Same as the train set of Camelyon17;
    \item \textbf{OOD val.}: Same as the validation set of Camelyon17;
    \item \textbf{OOD train}: Contains 10\% of the data from the test set;% of Camelyon17;
    \item \textbf{OOD test}: Contains the held-out 90\% of test data.% Camelyon17 test set.
\end{itemize}
%
Similar to our previous experiments, we train the linear heads on ID train and OOD train respectively, and evaluate all models on the OOD test set. 
%
We use 10-fold cross-validation for the OOD train and test set.
%
Following WILDS, we adopt DenseNet-121 \citep{dense} as backbone for all models, and the OOD validation set is used to perform early stopping and hyperparameter search.
%
The main results are shown in \cref{fig:camelyon,fig:camelyon_summary} and we provide more detailed numerical results with standard deviation values in \cref{tab:camelyon_std}.

\begin{table}
\parbox{.48\linewidth}{
\centering
\caption{Evaluations on test set of Camelyon17, all metrics computed using average accuracy.}
\vspace*{-0.8\baselineskip}
\scalebox{0.7}{
\begin{tabular}{llccc}    \toprule
    \multirow{2}{*}{Regime} &\multirow{2}{*}{Method} & \multicolumn{3}{c}{Metrics (\%)} \\
    \cmidrule{3-5} 
    & &  $\text{acc}_o(f,c_o)\uparrow$ & $\rho \downarrow$ & $b$ \\
    \midrule \rowcolor{lb}
    & AE          & 84.4 \std{2e+0} &-0.6 \std{1e+0}  &12.7 \std{2e+0} \\  \rowcolor{lb}
    & VAE         & 88.1 \std{2e+0} &  0.5 \std{2e+0} &39.0 \std{2e+0} \\  \rowcolor{lb}
    & IWAE        & 88.1 \std{1e+0} &-0.9 \std{3e+0}  &39.1 \std{4e+0} \\  \rowcolor{lb}
    \multirow{-4}{*}{AE}
    & $\beta$-VAE & 87.1 \std{4e+0} & 0.2 \std{4e+0} & 36.0 \std{5e+0} \\  \rowcolor{db}
    \multicolumn{2}{l}{\emph{\textbf{AE average}}} & \emph{86.9 \std{2e+0}}  & \emph{\textbf{-0.2 \std{3e+0}}}  & \emph{31.7 \std{3e+0}} \\
    \midrule \rowcolor{lg}
    & SimCLR      & 92.7 \std{2e+0} &  0.4 \std{1e+0} & 8.3 \std{1e+0} \\ \rowcolor{lg}
    & SimSiam     & 86.7 \std{1e+0} & 3.1 \std{1e+0} & 7.9 \std{3e+0}\\  \rowcolor{lg}
    \multirow{-3}{*}{SSL} 
    & BYOL        & 89.9 \std{1e+0} & 1.4 \std{1e+0} & 10.3 \std{2e+0}\\  \rowcolor{dg}
    \multicolumn{2}{l}{\emph{\textbf{SSL average}}} & \emph{\textbf{89.8 \std{1e+0}}} & \emph{1.6 \std{1e+0}} & \emph{8.8 \std{2e+0}}\\
    \midrule \rowcolor{g}
    SL
    & Supervised  & 86.8 \std{2e+0} & 3.5 \std{1e+0} &  7.4 \std{3e+0} \\ 
    \bottomrule
\end{tabular}
\label{tab:camelyon17_results}}
}
\hspace{10pt}
\parbox{.48\linewidth}{
\centering
\caption{Evaluations on test set of FMoW, all metrics computed using worst-group accuracy.}
\vspace*{-0.8\baselineskip}
\scalebox{0.7}{
\begin{tabular}{llccc}    \toprule
    \multirow{2}{*}{Regime} &\multirow{2}{*}{Method} & \multicolumn{3}{c}{Metrics (\%)} \\
    \cmidrule{3-5} 
    & &  $\text{acc}_o(f,c_o)\uparrow$ & $\rho \downarrow$ & $b$ \\
    \midrule \rowcolor{lb}
    & AE          & 26.9 \std{9e-3} & 6.4 \std{6e-3}  & 5.8 \std{1e-2} \\  \rowcolor{lb}
    & VAE         & 21.7 \std{6e-3} &  4.7 \std{4e-3} & 8.0 \std{2e-2} \\  \rowcolor{lb}
    & IWAE        & 20.9 \std{2e-2} & 5.5 \std{1e-2}  & 7.8 \std{1e-2} \\  \rowcolor{lb}
    \multirow{-4}{*}{AE}
    & $\beta$-VAE & 21.7 \std{5e-3} & 3.4 \std{6e-3} & 7.6  \std{8e-3} \\  \rowcolor{db}
    \multicolumn{2}{l}{\emph{\textbf{AE average}}} & \emph{22.8 \std{3e-2}}  & \emph{\textbf{5.0  \std{7e-3}}}  & \emph{7.3  \std{1e-2}} \\
    \midrule \rowcolor{lg}
    & SimCLR      & 29.9 \std{6e-3} &  10.7 \std{6e-3} & 7.6 \std{7e-3} \\ \rowcolor{lg}
    & SimSiam     & 27.8 \std{2e-2} & 4.6 \std{1e-2} & 6.3 \std{2e-2}\\  \rowcolor{lg}
    \multirow{-3}{*}{SSL} 
    & BYOL        & 31.3 \std{1e-2} & 12.1 \std{7e-3} & 7.9  \std{1e-2}\\  \rowcolor{dg}
    \multicolumn{2}{l}{\emph{\textbf{SSL average}}} & \emph{29.6 \std{2e-2}} & \emph{9.1 \std{9e-3}} & \emph{7.3 \std{1e-2}}\\
    \midrule \rowcolor{g}
    SL
    & Supervised  & \textbf{35.6 \std{7e-3}} & 37.7 \std{4e-2} &  6.9 \std{9e-3} \\ 
    \bottomrule
\end{tabular}
\label{tab:fmow_results}}
}
\end{table}






With the linear head trained on ID data, the left subplots in ~\Cref{fig:camelyon,fig:camelyon_summary} show that representations learned using SSL algorithms result in similar OOD test accuracy as those trained using SL, while the OOD accuracy from AE models is $\~10$ percentage points lower.
%This indicates that representations learned using SSL and SL are more robust to spurious correlations, as they perform better on OOD data than the AE models.

% With linear head trained on ID data~\Cref{fig:camelyon,fig:camelyon_summary}~(left) show that representations learning using SSL models on average achieve similar performance to the SL model, while AE models' accuracy on OOD test set is $\~10\%$ lower.
%
However, the OOD test accuracy of AE algorithms catches up to those from SL and SSL algorithms when we use the OOD linear head for evaluation. 
%
~\Cref{fig:camelyon_summary,fig:camelyon} (right subplots) show that SSL models achieve the best performance, out-performing AE and SL by nearly $3$ percentage points.
%
This demonstrates that the representations learned by SSL models are more robust against distribution shift than AE and SL models, which highlights a surprising adverse effect of labels for OOD generalisation in this setting.
%
Another significant finding of this experiment is that by using only $10\%$ of the data from the original test split to train the linear classification head, we are able to improve the performance of all models by $13$ percentage points on average.
%
All of this shows that the bias of the linear classification head plays a significant role even for real world distribution shifts, and that it is possible to mitigate this effect by training the linear head using a small amount of OOD data.

\subsection{Camelyon17\_SB}
%
To further examine models' ability to generalise OOD, we adjust the subpopulation of the training split of the Camelyon17 dataset to create a {\em simplicity bias} version of this realistic dataset.
%
Specifically, the ID train split of Camelyon17 contains tissue scans from 3 hospitals, that are labelled as either "benign" or "malignant".
%
To construct the train set of Camelyon17\_SB, we take only the "benign" samples from hospital 1 and 2, and only the "malignant" samples from hospital 3.
%
As such, the label and domain of examples in the train set are spuriously correlated.
%
Given the texture bias of CNNs \citep{texture1,texture2}, the model is prone to trivially minimising the training loss by using only domain information for classification, which would result in poor OOD generalisation performance.
%
Using the same experimental setup as in \cref{sec:camelyon17}, we report the results for Camelyon17\_SB in \cref{fig:camelyon_sb_summary,fig:camelyon_sb}.

Comparing the performance of models on the biased version of Camelyon17 (\Cref{fig:camelyon_sb_summary,fig:camelyon_sb}) to the performance on the original dataset (\Cref{fig:camelyon_summary,fig:camelyon}), we see that surprisingly, AE models experience almost no performance drop for both the ID and OOD linear head evaluation;
%
SL model, on the other hand, sees the most significant decline in its OOD generalisation performance, showing a 22\% accuracy decrease with ID linear head and 13\% with OOD linear head.
%
Additionally, consistent to our previous findings, unsupervised models (AE, SSL) outperforms supervised model (SL) on this dataset.
%
We also note that while with the original Camelyon17 dataset, SL model's performance catches up with the rest when using OOD linear head for evaluation, on Camelyon17\_SB there still exist a 10\% performance gap between SL and other unsupervised models when switching to OOD linear head.
%
The results further demonstrate that unsupervised models including AE and SSL are better at OOD generalisation than SL models, and their advantages become even more significant under this more challenging distribution shift setting.

==> 5relatedwork_v1.tex <==
\section{Related Work}

\paragraph{Learning with explicit distribution shift} 
%
Refers to when the features that caused distribution shift is explicit, known, controllable, and in some cases, extreme (e.g. MNIST-CIFAR, CdSprites).
%
This type of settings are popular in works that investigate simplicity bias \citep{neyshabur2014search, shah2020pitfalls}, dataset bias \citep{torralba2011datasetbias1} and shortcut learning \citep{geirhos2020shortcut, lapuschkin2019shortcut2}, as it allows for users to easily adjust the level of distribution shift between train and test set.
%
Various specialised methods that either mitigate or address these problems under the supervised learning regime have been proposed, including \citet{teney2022evading} that proposes to find shortcut solutions by ensembles, \citet{luo2021rectifying} that avoids shortcut learning by extracting foreground objects for representation learning only, as well as \citet{torralba2011datasetbias1, kim2019datasetbias2, le2020datasetbias3} that re-sample the dataset to reduce the spurious correlation. 


Importantly \citet{kirichenko2022last, kang2019decoupling} shows that this extreme simplicity bias can be mitigated in some cases by retraining the final linear layer.
%
This is a game changer, as it for the first time decouples the bias of the linear head from that of the main representation learning model.
%
Interestingly, \citet{robinson2021simplicity} also investigates the robustness of contrastive-SSL methods against simplicity bias. However, without training the linear head on OOD data, their finding is opposite to ours --- that SSL methods are not able to avoid shortcut solutions.


\paragraph{Domain generalisation}
%
Domain generalisation (DG) typically study distribution shifts that are implicit and hard to define (e.g. DomainNet, Office-Home, WILDS-Camelyon17).
%
In this regime, the training data are sampled from multiple domains, while data from a new target domain is used as test set.
%
In contrast to domain adaptation (DA), DG does not have access to unlabelled data from the target domain.
%
There are mainly two lines of work in DG, namely
%
1) \textit{Distributional Robustness approaches (DRO)}, which minimises the worst group accuracy to address covariate shift \citep{gretton2008covariate,gretton2009covariate} and subpopulation shift \citep{Sagawa2020dro, groupdro0hu};
%
2) \textit{Domain invariance}, which consists of methods that directly learn representations that are invariant across domains  \citep{ben2010theory,ganin2016dann,wang2019learning}, encourage the alignment of gradients from different domains \citep{koyama2021out,lopez-paz2017gradient,fish}, or optimise for representations that result in the same optimal classifier for different domains \citep{arjovsky2019irm}.
%
Apart from these supervised learning methods, the recent advancement of SSL has also inspired works in unsupervised domain generalisation \citep{zhang2022towards, harary2022unsupervised}.
%
While all these methods achieved impressive performance, we note that they are all specially designed for DG with the majority of the methods relying on domain information and label information.
%
In contrast, our work studies how existing standard representation learning methods such as SSL and AE performs on DG tasks, with none of the methods relying on human annotations.



\paragraph{Other studies on distribution shift of non-specialised methods}
%
While we are the first to systematically evaluate the OOD generalisation performance of different unsupervised learning objectives, there are other insightful work that considers important deep learning characteristics such as training procedure and architecture.
%
\citet{liu2022empirical} studies the impact of different pre-training set-ups to distribution shift robustness, including pre-training dataset, objective and data augmentation.
%
\citet{ghosal2022vision} focuses on architecture, and found that Vision Transformers are more robust to spurious correlations than ConvNets when using larger models and are given more training data;
%
further, \citet{liu2021self} found that SSL is more robust to data imbalance.
%
\citet{azizi2022robust} also performed extensive studies on the generalisation performance of SSL algorithms in medical data.
%
In contrast, our work investigates the distribution shift performance of both SSL and AE under synthetic and realistic settings; we do not consider the pre-training step, and focus instead on the training objectives.
%
Our experiments also go beyond the data imbalance setting and investigate a diverse range of distribution shift problems.

